Neural Point-Based Graphics

We present a new point-based approach for modeling the appearance of real scenes. The approach uses a raw point cloud as the geometric representation of a scene, and augments each point with a learnable neural descriptor that encodes local geometry and appearance. A deep rendering network is learned in parallel with the descriptors, so that new views of the scene can be obtained by passing the rasterizations of a point cloud from new viewpoints through this network. The input rasterizations use the learned descriptors as point pseudo-colors. We show that the proposed approach can be used for modeling complex scenes and obtaining their photorealistic views, while avoiding explicit surface estimation and meshing. In particular, compelling results are obtained for scene scanned using hand-held commodity RGB-D sensors as well as standard RGB cameras even in the presence of objects that are challenging for standard mesh-based modeling.

==> conclusion.tex <==
\section{Discussion}
\label{sect:discussion}

We have presented a neural point-based approach for modeling complex scenes. Similarly to classical point-based approaches, ours uses 3D points as modeling primitives. Each of the points in our approach is associated with a local descriptor containing information about local geometry and appearance. A rendering network that translates point rasterizations into realistic views, while taking the learned descriptors as an input point pseudo-colors. 
We thus demonstrate that point clouds can be successfully used as geometric proxies for neural rendering, while missing information about connectivity as well as geometric noise and holes can be handled by deep rendering networks gracefully. Thus, our method achieves similar rendering quality to mesh-based analog~\cite{Thies19}, surpassing it wherever meshing is problematic (e.g.~thin parts).

%The learning process is performed using a dataset of point clouds and images. After learning, our model can be fitted to new scenes and is capable of producing realistic views from new viewpoints. Notably, our system accomplishes this in a purely data-driven manner, while avoiding meshing, or any other form of explicit surface reconstruction, as well as without performing explicit geometric and photometric surface parameter estimation.

{\bf Limitations and further work.} Our model currently cannot fill very big holes in geometry in a realistic way. Such ability is likely to come with additional point cloud processing/inpainting that could potentially be trained jointly with our modeling pipeline. We have also not investigated the performance of the system for dynamic scenes (including both motion and relighting scenarios), where some update mechanism for the neural descriptors of points would need to be introduced. 

==> experiments.tex <==


\section{Experiments}


%\label{subsect:datasets}

\subsubsection{Datasets.} To demonstrate the versatility of the approach, we evaluate it on several types of real scenes. Thus, we consider three sources of data for our experiments. First, we take RGBD streams from the ScanNet dataset~\cite{Dai17b} of room-scale scenes scanned with a structured-light RGBD sensor\footnote{\texttt{https://structure.io/}}. Second, we consider RGB image datasets of still standing people captured by a mirrorless camera with high resolution (the views capture roughly 180 degrees). Finally, we consider two more scenes corresponding to two objects captured by a smartphone camera. $360^{\circ}$ camera flights of two selected objects (a potted plant and a small figurine) of a different kind captured from a circle around the object.  % Thus, we consider two types of capture. First, we consider RGBD streams from the ScanNet dataset~\cite{Dai17b} of room-scale scenes scanned with a structured-light RGBD sensor\footnote{\texttt{https://structure.io/}}. Second, we consider the RGB video streams captured by a camera. Finally, we demonstrate the relevance of our approach to modeling of photometrically-complex synthetic scenes by running it on a standard test scene from the Blender software~\cite{Blender}.

For all experiments, as per the two-stage learning scheme described in Sec.~\ref{subsect:learning}, we split the dataset into three parts, unless noted otherwise: \textbf{pretraining part}, \textbf{fine-tuning part}, and \textbf{holdout part}. The pretraining part contains a set of scenes, to which we fit the rendering network (alongside point descriptors). The fine-tuning part contains a subset of frames of a new scene, which are fitted by the model creation process started with pretrained weights of the rendering network. The holdout part contains additional views of the new scene that are not shown during fitting and are used to evaluate the performance.

% For the ScanNet scenes, we use the provided registration data obtained with the BundleFusion~\cite{Dai17a} method. We also use the mesh geometry computed by BundleFusion in mesh-based baselines. Given the registration data, point clouds are obtained by joining together the 3D points from all RGBD frames and using volumetric subsampling (with the grid step 1 cm) resulting in the point clouds containing few million points per scene. In the evaluation, we use two ScanNet scenes '\textbf{Studio}' (scene 0), which has 5578 frames, and '\textbf{LivingRoom}' (scene 24), which has 3300 frames. In each case, we use every 100th frame in the trajectory for validation and remove 20 preceding and 20 following frames from each of these validation frames from the fitting set, using remaining 2202 and 1287 frames respectively for the fitting (fine-tuning) and descriptor estimation. We pretrain rendering networks on the set of 100 scenes (preprocessed in a similar fashion) that does not include Studio and LivingRoom scenes.

For the ScanNet scenes, we use the provided registration data obtained with the BundleFusion~\cite{Dai17a} method. We also use the mesh geometry computed by BundleFusion in mesh-based baselines. Given the registration data, point clouds are obtained by joining together the 3D points from all RGBD frames and using volumetric subsampling (with the grid step 1 cm) resulting in the point clouds containing few million points per scene. We pretrain rendering networks on a set of 100 ScanNet scenes. In the evaluation, we use two ScanNet scenes '\textbf{Studio}' (scene 0), which has 5578 frames, and '\textbf{LivingRoom}' (scene 24), which has 3300 frames (both scenes are not from the pretraining part). In each case, we use every $100^{\text{th}}$ frame in the trajectory for holdout and, prior to the fitting, we remove 20 preceding and 20 following frames for each of the holdout frames from the fine-tuning part to ensure that holdout views are sufficiently distinct.% , using remaining 2202 and 1287 frames respectively for the fitting (fine-tuning) and descriptor estimation.

\begin{figure}[!h]
    \centering
    % \begin{subfigure}{.11\textwidth}
    %     \includegraphics[width=\textwidth]{figures/various_people/DSC03446.jpg}
    % \end{subfigure}
    \begin{subfigure}{.135\textwidth}
        \includegraphics[width=\textwidth]{figures/various_people/DSC03575.jpg}
    \end{subfigure}
    % \begin{subfigure}{.09\textwidth}
    %     \includegraphics[width=\textwidth]{figures/various_people/DSC03948.jpg}
    % \end{subfigure}
    \begin{subfigure}{.135\textwidth}
        \includegraphics[width=\textwidth]{figures/various_people/DSC04590.jpg}
    \end{subfigure}
    % \begin{subfigure}{.09\textwidth}
    %     \includegraphics[width=\textwidth]{figures/various_people/DSC04609.jpg}
    % \end{subfigure}
    \begin{subfigure}{.135\textwidth}
        \includegraphics[width=\textwidth]{figures/various_people/DSC05393.jpg}
    \end{subfigure}
    \begin{subfigure}{.135\textwidth}
        \includegraphics[width=\textwidth]{figures/various_people/DSC05635.jpg}
    \end{subfigure}
    % \begin{subfigure}{.09\textwidth}
    %     \includegraphics[width=\textwidth]{figures/various_people/DSC05780.jpg}
    % \end{subfigure}
    \begin{subfigure}{.135\textwidth}
        \includegraphics[width=\textwidth]{figures/various_people/DSC07476.jpg}
    \end{subfigure}
    \begin{subfigure}{.135\textwidth}
        \includegraphics[width=\textwidth]{figures/various_people/DSC07654.jpg}
    \end{subfigure}
    \begin{subfigure}{.135\textwidth}
        \includegraphics[width=\textwidth]{figures/various_people/DSC09456.jpg}
    \end{subfigure}
    \caption{Representative samples from the People dataset used in our experiments.}
    \label{fig:people-various}
\end{figure}


% For the smartphone-captured scenes, we have run the commercial Agisoft~Metashape~\cite{agisoft} package, which is one of the best packages for scene modeling/reconstruction. Agisoft Metashape provides the registration, the point cloud, and the mesh by running proprietary structure-and-motion and dense multiview stereo methods. We evaluate on two scenes: '\textbf{Shoe}' and '\textbf{Plant}'. The plant scene contains 2727 frames taken with 250ms intervals, out of which we put every 50th into the validation set and withhold 10 frames around these frames and use the rest as the fitting set. The \textit{shoe} scene has been taken deliberately very small number of images, as it contains 100 frames taken with 250ms intervals, which we shuffle and hold out 10 frames for validation.

% For the camera-captured scenes, we collected 123 sequences of 41 distinct people, each in 3 different predefined poses, by a Sony a7-III mirrorless camera. Each person was asked to stand still (like a mannequin) against a white wall for 30--45 seconds and was photographed by a slowly moving camera along a continuous trajectory, every time chosen randomly such that the camera perceives the frontal half of a body, head, and hair from several angles. Background was removed on all images by a human segmentation network~\cite{Gong19} (authors-provided implementation was used), and the obtained sequences were processed by a commercial off-the-shelf Agisoft~Metashape~\cite{agisoft} package. Agisoft~Metashape provides a registration, a point cloud, and a mesh by running proprietary structure-and-motion and dense multiview stereo methods. Videos of all people were taken under artificial light in $6\text{K} \times 4\text{K}$ pixels resolution in continuous shooting mode yielding 150--200 frames per sequence, with camera parameters selected in a balanced manner (ISO 2500, F9, and 1/400 s shutter speed), and subsequently bilinearly downsampled to 4K resolution (on the long side) for processing. Human segmentation network was operating on images downsampled to 1200 pixels (on the long side) due to the GPU memory limitation. Later on, we will refer to this data as People dataset. In addition, we captured $360^{\circ}$ video sequences of two scenes of a different kind --- '\textbf{Owl}' and '\textbf{Plant}' --- by a commodity-level smartphone. These objects feature materials and structures with different properties, and this is of interest whether the method can generalize to these complications. TODO INFO ABOUT OWL AND PLANT, NUMBER OF FRAMES, ETC. % The plant scene contains 2727 frames taken with 250ms intervals, out of which we put every 50th into the validation set and withhold 10 frames around these frames and use the rest as the fitting set. % The \textit{TODO OWL?} scene has been taken deliberately very small number of images, as it contains 100 frames taken with 250ms intervals, which we shuffle and hold out 10 frames for validation.

For the camera-captured scenes of humans, we collected 123 sequences of 41 distinct people, each in 3 different poses, by a Sony a7-III mirrorless camera. Each person was asked to stand still (like a mannequin) against a white wall for 30--45 seconds and was photographed by a slowly moving camera along a continuous trajectory, covering the frontal half of a body, head, and hair from several angles. We then remove (whiten) the backround using the method~\cite{Gong19}, and the result is processed by the Agisoft~Metashape~\cite{agisoft} package that provides camera registration, the point cloud, and the mesh by running proprietary structure-from-motion and dense multiview stereo methods. Each sequence contains 150-200 ten megapixel frames with high amount of fine details and varying clothing and hair style (Fig.~\ref{fig:people-various}). The pretraining set has 102 sequences of 38 individuals, and three scenes of three different individuals were left for validation. Each of the validation scenes is split into fine-tuning (90\% of frames) and holdout (10\% of frames) sets randomly.

In addition, we used a smartphone (Galaxy S10e) to capture $360^{\circ}$ sequences of two scenes containing an \textbf{Owl} figurine (61 images) and a potted \textbf{Plant} (92 images). All frames of both scenes were segmented manually via tools from Adobe Photoshop CC software package. We split fine-tuning and holdout parts in the same manner as in People dataset.


% \begin{figure*}
%     \captionsetup[subfigure]{labelformat=empty}
      
%       \begin{subfigure}{0.32\linewidth}
%       \includegraphics[width=\textwidth]{figures/scannet_studio_00/2500_deferred_full.png}
%       \end{subfigure}
%       \begin{subfigure}{0.32\linewidth}
%       \includegraphics[width=\textwidth]{figures/scannet_studio_00/2500_ours_full.png}
%       \end{subfigure}
%       \begin{subfigure}{0.32\linewidth}
%       \includegraphics[width=\textwidth]{figures/scannet_studio_00/2500_gt_full.png}
%       \end{subfigure}
      
%       \begin{subfigure}{0.32\linewidth}
%       \includegraphics[width=\textwidth]{figures/scannet_studio_00/0_deferred_full.png}
%       \caption{Deferred Neural Rendering}
%       \end{subfigure}
%       \begin{subfigure}{0.32\linewidth}
%       \includegraphics[width=\textwidth]{figures/scannet_studio_00/0_ours_full.png}
%       \caption{Ours}
%       \end{subfigure}
%       \begin{subfigure}{0.32\linewidth}
%       \includegraphics[width=\textwidth]{figures/scannet_studio_00/0_gt_full.png}
%       \caption{Ground truth}
%       \end{subfigure}
      
%     \caption{Comparative results on the 'Studio' dataset (from \cite{Dai17b}). We show the textured mesh, the colored point cloud, the results of three neural rendering systems (including ours), and the ground truth. Our system can successfully reproduce details that pose challenging for meshing, and suffers less from blurriness than the Direct RenderNet system.} 
%     \label{fig:studio}
% \end{figure*}

\begin{figure*}[!h]
    \centering
    \captionsetup[subfigure]{labelformat=empty}
      \begin{subfigure}{0.18\linewidth}
      \includegraphics[trim={0 0 12.5cm 0}, clip,width=\linewidth]{figures/scannet_studio_00/2500_pc_ps4.jpg}
      \end{subfigure}
      \begin{subfigure}{0.18\linewidth}
      \includegraphics[trim={0 0 12.5cm 0}, clip,width=\linewidth]{figures/scannet_studio_00/2500_gray.jpg}
      \end{subfigure}
      \begin{subfigure}{0.18\linewidth}
      \includegraphics[trim={0 0 12.5cm 0}, clip,width=\linewidth]{figures/scannet_studio_00/2500_deferred.jpg}
      \end{subfigure}
      \begin{subfigure}{0.18\linewidth}
      \includegraphics[trim={0 0 12.5cm 0}, clip,width=\linewidth]{figures/scannet_studio_00/2500_ours.jpg}
      \end{subfigure}
      \begin{subfigure}{0.18\linewidth}
      \includegraphics[trim={0 0.25cm 9.5cm 0}, clip,width=\linewidth]{figures/scannet_studio_00/2500_nearest.jpg}
      \end{subfigure}
      \hfill
      \begin{subfigure}{0.18\linewidth}
      \includegraphics[trim={5cm 0 7.5cm 0}, clip,width=\linewidth]{figures/scannet_studio_00/novel_pc.jpg}
      \caption{Point Cloud}
      \end{subfigure}
      \begin{subfigure}{0.18\linewidth}
      \includegraphics[trim={5cm 0 7.5cm 0}, clip,width=\linewidth]{figures/scannet_studio_00/novel_mesh.jpg}
      \caption{Mesh}
      \end{subfigure}
      \begin{subfigure}{0.18\linewidth}
      \includegraphics[trim={5cm 0 7.5cm 0}, clip,width=\linewidth]{figures/scannet_studio_00/novel_deferred.jpg}
      \caption{DNR}
      \end{subfigure}
      \begin{subfigure}{0.18\linewidth}
      \includegraphics[trim={5cm 0 7.5cm 0}, clip,width=\linewidth]{figures/scannet_studio_00/novel_ours.jpg}
      \caption{Ours}
      \end{subfigure}
      \begin{subfigure}{0.18\linewidth}
      \includegraphics[trim={8.5cm 0.25cm 1cm 0}, clip,width=\linewidth]{figures/scannet_studio_00/novel_nearest.jpg}
      \caption{Nearest train}
      \end{subfigure}
    \caption{Comparative results on the 'Studio' dataset (from \cite{Dai17b}). We show the textured mesh, the colored point cloud, the results of three neural rendering systems (including ours), and the ground truth. Our system can successfully reproduce details that pose challenge for meshing, such as the wheel of the bicycle.} 
    \label{fig:studio-holdout}
\end{figure*}


\begin{figure*}[!h]
      %\rotatebox{90}{Person 1}
      \centering
      \begin{subfigure}[c]{0.23\textwidth}
      \centering
      \includegraphics[width=\linewidth]{figures/Olya/DSC09255_ours_full.jpg}
      \end{subfigure}
       \hfill
      \begin{subfigure}[c]{0.23\textwidth}
      \centering
      \includegraphics[width=\linewidth]{figures/Olya/DSC09255_gt_full.jpg}
      \end{subfigure}
       \hfill
      %\rotatebox{90}{Person 1}
      \begin{subfigure}[c]{0.23\textwidth}
      \centering
      \includegraphics[width=\linewidth]{figures/Olya/DSC09238_ours_full.jpg}
      %\caption{Ours}
      \end{subfigure}
      \hfill
      \begin{subfigure}[c]{0.23\textwidth}
      \centering
      \includegraphics[width=\linewidth]{figures/Olya/DSC09238_gt_full.jpg}
      %\caption{Ground truth}
      \end{subfigure}
    %   \hfill
      
      \medskip
      %\rotatebox{90}{Person 2}
      \begin{subfigure}[c]{0.23\textwidth}
      \centering
      \includegraphics[width=\linewidth]{figures/Egor/DSC06090_ours_full.jpg}
      \caption*{Ours}
      \end{subfigure}
       \hfill
      \begin{subfigure}[c]{0.23\textwidth}
      \centering
      \includegraphics[width=\linewidth]{figures/Egor/DSC06090_gt_full.jpg}
      \caption*{Ground truth}
      \end{subfigure}
       \hfill
      % \rotatebox{90}{Person 2}
      \begin{subfigure}[c]{0.23\textwidth}
      \centering
      \includegraphics[width=\linewidth]{figures/Egor/DSC06150_ours_full.jpg}
      \caption*{Ours}
      \end{subfigure}
       \hfill
      \begin{subfigure}[c]{0.23\textwidth}
      \centering
      \includegraphics[width=\linewidth]{figures/Egor/DSC06150_gt_full.jpg}
      \caption*{Ground truth}
      \end{subfigure}
      %\hfill
    \caption{Results on the holdout frames from the 'Person 1' and 'Person 2' scenes. Our approach successfully transfers fine details to new views.}
    \label{fig:people-holdout}
\end{figure*}

% \begin{figure*}
%     \captionsetup[subfigure]{labelformat=empty}
      
%       \begin{subfigure}{0.32\linewidth}
%       %\includegraphics[width=\textwidth]{figures/comparison/scene0000_val/3300_texture_stack.png}
%       \caption{Deferred Neural Rendering}
%       \end{subfigure}
%       \begin{subfigure}{0.32\linewidth}
%       %\includegraphics[width=\textwidth]{figures/comparison/scene0000_val/3300_pcd_stack.png}
%       \caption{Ours}
%       \end{subfigure}Fig. 4: Comparative results on the ’Plant’ scene – same format as in Figure 2.

%       \begin{subfigure}{0.32\linewidth}
%       %\includegraphics[width=\textwidth]{figures/comparison/scene0000_val/3300_pix2pix_stack.png}
%       \caption{Ground truth}
%       \end{subfigure}
      
%     \caption{Comparative results on the 'LivingRoom' scene (from \cite{Dai17b}) -- same format as in \fig{studio}.}
%     \label{fig:living}
% \end{figure*}
      
\begin{figure*}[!h]
    %\captionsetup[subfigure]{labelformat=empty}
      \rotatebox{90}{Plant}
      \begin{subfigure}{0.32\linewidth}
      \includegraphics[width=\textwidth]{figures/plant/0026_pc_full.jpg}
      \caption{Point cloud}
      \end{subfigure}
      \begin{subfigure}{0.32\linewidth}
      \includegraphics[width=\textwidth]{figures/plant/0026_mesh_full.jpg}
      \caption{Mesh+Texture}
      \end{subfigure}
      \begin{subfigure}{0.32\linewidth}
      \includegraphics[width=\textwidth]{figures/plant/0026_pix2pix_full.jpg}
      \caption{Pix2Pix}
      \end{subfigure}
      
      \rotatebox{90}{Plant}
      \begin{subfigure}{0.32\linewidth}
      \includegraphics[width=\textwidth]{figures/plant/0026_deferred_full.jpg}
      \caption{Deferred Neural Rendering}
      \end{subfigure}
      \begin{subfigure}{0.32\linewidth}
      \includegraphics[width=\textwidth]{figures/plant/0026_ours_full.jpg}
      \caption{Ours}
      \end{subfigure}
      \begin{subfigure}{0.32\linewidth}
      \includegraphics[width=\textwidth]{figures/plant/0026_gt_full.jpg}
      \caption{Ground truth}
      \end{subfigure}
    
    %   \rotatebox{90}{Owl}
    %   \begin{subfigure}{0.32\linewidth}
    %   \includegraphics[width=\textwidth]{figures/owl/0026_pc_full.png}
    %   \caption{Point cloud}
    %   \end{subfigure}
    %   \begin{subfigure}{0.32\linewidth}
    %   \includegraphics[width=\textwidth]{figures/owl/0026_mesh_full.png}
    %   \caption{Mesh+Texture}
    %   \end{subfigure}
    %   \begin{subfigure}{0.32\linewidth}
    %   \includegraphics[width=\textwidth]{figures/owl/0026_pix2pix_full.png}
    %   \caption{Direct RenderNet}
    %   \end{subfigure}
      
    %   \rotatebox{90}{Owl}
    %   \begin{subfigure}{0.32\linewidth}
    %   \includegraphics[width=\textwidth]{figures/owl/0026_deferred_full.png}
    %   \caption{Deferred Neural Rendering}
    %   \end{subfigure}
    %   \begin{subfigure}{0.32\linewidth}
    %   \includegraphics[width=\textwidth]{figures/owl/0026_ours_full.png}
    %   \caption{Ours}
    %   \end{subfigure}
    %   \begin{subfigure}{0.32\linewidth}
    %   \includegraphics[width=\textwidth]{figures/owl/0026_gt_full.png}
    %   \caption{Ground truth}
    %   \end{subfigure}
    \caption{Comparative results on the holdout frame from the 'Plant' scene. Our method better preserves thin parts of the scene.}
    \label{fig:plant-holdout}
\end{figure*}


%Videos of all people were taken under artificial light in $6\text{K} \times 4\text{K}$ resolution with 150--200 frames per sequence, and subsequently bilinearly downsampled to 4K resolution (on the long side) for processing. Human segmentation network was operating on images downsampled to 1200 pixels on the long side. Professional camera with high level of detailization was used to capture the source sequences for this dataset in order to test the applicability of the method to rendering of subtle details of human face, hair, and clothing. Later on, we will refer to this data as \textbf{People} dataset. 102 scenes of 38 people were selected for the network pretraining, and the remaining 3 people were selected for validation. In particular, we take one scene of each of the 3 people, and split it in a fine-tuning and holdout parts (in 90\%/10\% proportion of randomly shuffled frames) for 3 separate quality tests.




% We use the ScanNet dataset~\cite{Dai17b}, which is a collection of room-scale scans with available raw RGBD data streams, their camera registration parameters, as well as surface meshes reconstructed using the BundleFusion algorithm~\cite{Dai17a}, which we use for mesh-based baselines.

% We use a set of 52 scenes for the training of our system. To obtain the point cloud geometry, we combine the depth scans using camera intrinsic and extrinsic parameters provided by Scannet. To reduce the number of points in point clouds we apply volumetric subsampling (with the grid step 10cm) and apply a small jitter to point coordinates. Jitter helps to destroy regular pattern in a subsampled point cloud, which becomes apparent on a 2D projection. Typically, the number of points in a scene is between 1 and 10 millions of points after subsampling.

% The evaluation is performed on two hold-out scenes from Scannet, namely on scene-0 and scene-24. Additionally we use two scenes, a plant and a shoe, created from RGB videos taken from a modern smartphone (Samsung Galaxy S10). We use the commercial off-the-shelf software package~\cite{AgiSoft} to obtain the registration, the point cloud as well as the reconstructed mesh with texture.

% In the scene-00, the whole trajectory of the camera includes 5578 frames, of which we put every 100th into the validation set. We then withhold the temporal window of 20 frames around each of the validation frames and use the remaining 3303 frames for learning/fine-tuning of our method as well as the baseline methods. For splitting scene-24 on train and validations sets we use the same approach as with the scene-00 and have 2007 frames for training out of 3398 frames. The plant scene contains 2727 frames taken with 250ms intervals, out of which we put every 50th into the validation set and withhold 10 frames around these frames and use the rest for the training set. The shoe scene contains 100 frames taken with 250ms intervals, which we shuffle and hold out 10\% for validation. 


% \begin{table*}
%     \centering
%     \begin{tabular}{|c|c|c|c|c|c|}
%     \hline
%          & Studio & LivingRoom & Shoe & Plant& \\
%     Method & (RGBD stream) & (RGBD stream) & (RGB video) & (RGB video) & RenderNet \\
%     & Loss$\downarrow$\; PSNR$\uparrow$\; SSIM$\uparrow$ & Loss$\downarrow$\; PSNR$\uparrow$\; SSIM$\uparrow$ & Loss$\downarrow$\; PSNR$\uparrow$\; SSIM$\uparrow$ & Loss$\downarrow$\; PSNR$\uparrow$\; SSIM$\uparrow$ & params\\
%     \hline
%     Mesh+texture & 551.193\;18.372\;0.821 & 678.957\;15.373\;0.764 & 378.502\;20.229\;0.852 & 482.707\;18.822\;0.746 & -\\
%     % Surface light field & TODO/TODO & TODO/TODO & 433\;20.3180\;0.8567 & 566.3137\;17.2121\;0.7187 & ?\\
%     Mesh+RenderNet & 539.210\;19.180\;0.840 & 581.367\;17.536\;0.819 & \textbf{280.242}\;\textbf{24.062}\;\textbf{0.910} & 375.322\;21.846\;\textbf{0.817} & 1.96M\\
%     Ours-scene & \textbf{523.287}\;\textbf{19.615}\;\textbf{0.841} & \textbf{545.406}\;\textbf{18.486}\;\textbf{0.828} & 284.617\;23.851\;0.888 & \textbf{340.275}\;\textbf{22.674}\;\textbf{0.817} & 1.96 M\\
%     \hline
%     *Direct RenderNet& 528.705\;18.185\;0.819 & 557.513\;16.840\;0.793 & 265.722\;22.552\;0.890 & 363.445\;21.888\;0.801 & 1.96 M\\
%     *Direct RenderNet (slow) & 518.310\;19.814\;0.850 & 534.648\;18.834\;0.840 & 260.530\;\textbf{25.936}\;\textbf{0.920} & 345.232\;23.334\;0.837 & \textit{7.84 M}\\    
%     *Ours-full & \textbf{508.182}\;19.899\;0.852 & \textbf{525.016}\;18.888\;\textbf{0.842} & 260.981\;25.330\;0.917 & \textbf{323.483}\;\textbf{23.655}\;\textbf{0.844} & 1.96 M\\
%     *Ours-universal & 510.135\;\textbf{19.900}\;\textbf{0.863} & 525.043\;\textbf{18.894}\;\textbf{0.842} & \textbf{259.528}\;25.524\;0.917 & \textbf{323.483}\;\textbf{23.655}\;\textbf{0.844} & 1.96 M\\
%     \hline

%     %Ours-full & 506.2007 & 526.2108 & 261.1608 & 326.1616 & ?\\
%     \end{tabular}
%     \caption{Comparison results in terms of the perceptual loss (lower is better), PSNR (higher is better), SSIM (higher is better) measures. The methods marked with $^*$ have been pretrained on a hold-out scene dataset. See text for the description of methods. In most cases and in most metrics, the variants of our method perform better.  }
%     \label{tab:comparison}
% \end{table*}

% \begin{table}[]
% \centering
% %\scriptsize
% \begin{tabular}{l|c|c|c|c|c|c|}
%                             & \multicolumn{6}{c|}{ScanNet scene}                                                                                \\ \cline{2-7} 
%                             & \multicolumn{3}{c|}{LivingRoom}                        & \multicolumn{3}{c|}{Studio}                              \\
% Method                      & VGG $\downarrow$ & LPIPS $\downarrow$ & IS $\uparrow$  & VGG  $\downarrow$ & LPIPS  $\downarrow$ & IS $\uparrow$  \\ \hline
% Direct RenderNet            & 751.04           & 0.564              & \textbf{4.000} & 633.30            & 0.535               & 4.795          \\
% Direct RenderNet (slow)     & 741.09           & 0.547              & 3.708          & 619.04            & 0.509               & 4.510          \\
% Neural Rerendering          & 751.52           & 0.580              & 3.641          & 634.93            & 0.529               & 4.941          \\
% Neural Rerendering (slow)   & 739.82           & 0.542              & 3.898          & 620.98            & 0.507               & 4.826          \\
% Textured mesh               & 791.26           & 0.535              & 3.614          & 690.67            & 0.540               & 5.203          \\
% Deferred Neural Rerendering & \textbf{725.23}  & 0.492              & 3.398          & 603.63            & 0.484               & 4.916          \\ \hline
% Ours                        & 727.38           & \textbf{0.488}     & 3.360          & \textbf{595.24}   & \textbf{0.472}      & \textbf{5.226}
% \end{tabular}
% \label{tab:comparison_scannet}
% \end{table}

\begin{table}[!h]
%\centering
\caption{Comparison with the state-of-the-art for all considered hold-out scenes from various sources: two scenes from ScanNet, two people captured by a professional camera, and two objects photographed by a smartphone. We assess all methods with respect to widely used perceptual metrics correlated with visual similarity of predicted and ground truth images (LPIPS, FID) and to VGG loss used in our experiments.}
\vspace{0.2cm}
\begin{subtable}{1\textwidth}
\begin{tabular}{r|c|c|c|c|c|c}
                            %& \multicolumn{6}{c|}{ScanNet scenes}  \\ 
                            %\cline{2-7} 
                            & \multicolumn{3}{c|}{ScanNet - LivingRoom}                                                       & \multicolumn{3}{c}{ScanNet - Studio}                                                           \\
Method                      & VGG $\downarrow$                 & LPIPS $\downarrow$              & FID $\downarrow$ & VGG  $\downarrow$                & LPIPS  $\downarrow$        & FID $\downarrow$ \\ \hline
Pix2Pix            & 751.04                           & 0.564                           & 192.82           & 633.30                           & 0.535                       & 127.49           \\
Pix2Pix (slow)     & 741.09                           & 0.547                           & 187.92           & 619.04                           & 0.509                      & 109.46           \\
Neural Rerendering          & 751.52                           & 0.580                           & 206.90           & 634.93                           & 0.529                      & 119.16           \\
Neural Rerendering (slow)   & 739.82                           & 0.542                           & 186.27           & 620.98                           & 0.507                      &  108.12       \\
Textured mesh               & 791.26                           & 0.535                           & 152.02            & 690.67                           & 0.540                     & 97.95           \\
Deferred Neural Rendering & \textbf{725.23}                     & 0.492                         & \textbf{129.33}   & 603.63                           & 0.484                      & 84.92  \\ \hline
%Ours (splatting)            & 726.50                           & \textbf{0.485}                 & 139.90            &\textbf{591.87}                & \textbf{0.470}                     & 81.94 \\
Ours                        & 727.38                           & \textbf{0.488}                          & 138.87            & \textbf{595.24}                   & \textbf{0.472}    & \textbf{76.73}          
\end{tabular}
\label{tab:comparison_scannet}
\end{subtable}

\vspace{0.2cm}
%\centering
\begin{subtable}{1\textwidth}
\begin{tabular}{r|c|c|c|c|c|c}
                          & \multicolumn{3}{c|}{People - Person 1}                            & \multicolumn{3}{c}{People - Person 2}                              \\
Method                    & VGG $\downarrow$ & LPIPS $\downarrow$ & FID $\downarrow$ & VGG  $\downarrow$ & LPIPS  $\downarrow$ & FID $\downarrow$ \\ \hline
Pix2Pix                   & 209.16           & 0.1016             & 51.38            & 186.89            & 0.1642              & 114.93           \\
Pix2Pix (slow)            & 204.45           & 0.0975             & 47.14            & 179.99            & 0.1566              & 102.62           \\
Textured mesh             & \textbf{155.37}  & 0.0698             & 60.62            & 163.73            & 0.1404              & 96.20            \\
Deferred Neural Rendering & 184.86           & 0.0659             & 34.41            & 163.13            & 0.1298              & 78.70            \\ \hline
%Ours (splatting)          & 186.06           & 0.0664             & 44.63            & 162.56            & 0.1174              & 80.60            \\
Ours                      & 181.11           & \textbf{0.0602}    & \textbf{32.63}   & \textbf{161.18}   & \textbf{0.1131}     & \textbf{77.92}  
\end{tabular}
\label{tab:comparison_people}
\end{subtable}

\vspace{0.2cm}
\begin{subtable}{1\textwidth}
\begin{tabular}{r|c|c|c|c|c|c}
                          & \multicolumn{3}{c|}{Plant}                               & \multicolumn{3}{c}{Owl}                                   \\
Method                    & VGG $\downarrow$ & LPIPS $\downarrow$ & FID $\downarrow$ & VGG  $\downarrow$ & LPIPS  $\downarrow$ & FID $\downarrow$ \\ \hline
Pix2Pix          & 85.47            & 0.0443             & 52.95            & 34.30             & 0.0158              & 124.63           \\
Pix2Pix (slow)   & 82.81            & 0.0422             & 48.89            & 32.93             & 0.0141              & 101.65           \\
Textured mesh             & 101.56           & 0.0484             & 95.60            & 36.58             & 0.0145              & 141.66           \\
Deferred Neural Rendering & 77.55            & 0.0377             & 49.61            & \textbf{28.12}             & \textbf{0.0096}              & \textbf{54.14}            \\ \hline
Ours                      & \textbf{75.08}            & \textbf{0.0373}             & \textbf{41.67}            & 29.69             & 0.0103              & 78.55           
\end{tabular}
\label{tab:comparison_things}
\end{subtable}
\label{tab:comparison_with_others}
\end{table}

% \begin{table}[]
% \centering
% \begin{tabular}{l|c|c|c|c|c|c|}
%                             & \multicolumn{6}{c|}{People}                                                                                 \\ \cline{2-7} 
%                             & \multicolumn{3}{c|}{Person 1}                            & \multicolumn{3}{c|}{Person 2}                              \\
% Method                      & VGG $\downarrow$ & LPIPS $\downarrow$ & FID $\downarrow$ & VGG  $\downarrow$ & LPIPS  $\downarrow$ & FID $\downarrow$ \\ \hline
% Direct RenderNet            & 209.16           & 0.1016             & 51.377           & 186.89            & 0.1642              & 114.932          \\
% Direct RenderNet (slow)     & 204.45           & 0.0975             & 47.143           & 179.99            & 0.1566              & 102.606          \\
% Textured mesh               & \textbf{168.10}  & 0.0675             & 59.045           & 177.65            & 0.1242              & 96.104           \\
% Deferred Neural Rendering & 184.86           & 0.0659             & 34.413           & 163.13            & 0.1298              & 78.702           \\ \hline
% Ours                        & 181.11           & \textbf{0.0602}    & \textbf{32.625}  & \textbf{161.18}   & \textbf{0.1131}     & \textbf{77.923} 
% \end{tabular}
% \label{tab:comparison_people}
% \end{table}

% \begin{table}[]
% \centering
% \begin{tabular}{l|c|c|c|c|}
%                             & \multicolumn{4}{c|}{Additional scenes}                                           \\ \cline{2-5} 
%                             & \multicolumn{2}{c|}{Plant}            & \multicolumn{2}{c|}{Owl}              \\
% Method                      & VGG $\downarrow$ & LPIPS $\downarrow$ & VGG  $\downarrow$ & LPIPS  $\downarrow$ \\ \hline
% Direct RenderNet            &                  &                    &                   &                     \\
% Direct RenderNet (slow)     &                  &                    &                   &                     \\
% Neural Rerendering          &                  &                    &                   &                     \\
% Neural Rerendering (slow)   &                  &                    &                   &                     \\
% Textured mesh               &                  &                    &                   &                     \\
% Deferred Neural Rendering & \textbf{}        &                    &                   &                     \\ \hline
% Ours                        &                  &                    &                   &                    
% \end{tabular}
% \label{tab:comparison_things}
% \end{table}

% \begin{figure*}[h!]
%     \captionsetup[subfigure]{labelformat=empty}

%       \begin{subfigure}{0.24\linewidth}
%       \includegraphics[width=\textwidth]{figures/comparison/bycicle/2448_texture_rect.png}
%       \end{subfigure}
%     %   \hspace*{0.05em}
%       \begin{subfigure}{0.24\linewidth}
%       \includegraphics[width=\textwidth]{figures/comparison/bycicle/2448_color_rect.png}  
%       \end{subfigure}
%       \begin{subfigure}{0.24\linewidth}
%       \includegraphics[width=\textwidth]{figures/comparison/bycicle/2448_pix2pix_rect.png} 
%       \end{subfigure}
%       \begin{subfigure}{0.24\linewidth}
%       \includegraphics[width=\textwidth]{figures/comparison/bycicle/2448_ours_rect.png}
%       \end{subfigure}
      
%       \begin{subfigure}{0.24\linewidth}
%       \includegraphics[width=\textwidth]{figures/comparison/bycicle/texture_stack.png}
%       \end{subfigure}
%     %   \hspace*{0.05em}
%       \begin{subfigure}{0.24\linewidth}
%       \includegraphics[width=\textwidth]{figures/comparison/bycicle/color_stack.png}  
%       \end{subfigure}
%       \begin{subfigure}{0.24\linewidth}
%       \includegraphics[width=\textwidth]{figures/comparison/bycicle/pix2pix_stack.png} 
%       \end{subfigure}
%       \begin{subfigure}{0.24\linewidth}
%       \includegraphics[width=\textwidth]{figures/comparison/bycicle/ours_stack.png}
%       \end{subfigure}
      
%       \begin{subfigure}{0.24\linewidth}
%       \includegraphics[width=\textwidth]{figures/comparison/scene0024_sofa/texture_rect.png}
%       \end{subfigure}
%     %   \hspace*{0.05em}
%       \begin{subfigure}{0.24\linewidth}
%       \includegraphics[width=\textwidth]{figures/comparison/scene0024_sofa/color_rect.png}
%       \end{subfigure}
%       \begin{subfigure}{0.24\linewidth}
%       \includegraphics[width=\textwidth]{figures/comparison/scene0024_sofa/pix2pix_rect.png}
%       \end{subfigure}
%       \begin{subfigure}{0.24\linewidth}
%       \includegraphics[width=\textwidth]{figures/comparison/scene0024_sofa/our_rect.png}
%       \end{subfigure}
      
%       \begin{subfigure}{0.24\linewidth}
%       \includegraphics[width=\textwidth]{figures/comparison/scene0024_sofa/texture_stack.png}
%       \caption{Mesh}
%       \end{subfigure}
%     %   \hspace*{0.05em}
%       \begin{subfigure}{0.24\linewidth}
%       \includegraphics[width=\textwidth]{figures/comparison/scene0024_sofa/color_stack.png}
%       \caption{Point cloud}
%       \end{subfigure}
%       \begin{subfigure}{0.24\linewidth}
%       \includegraphics[width=\textwidth]{figures/comparison/scene0024_sofa/pix2pix_stack.png}
%       \caption{DirectTranslation}
%       \end{subfigure}
%       \begin{subfigure}{0.24\linewidth}
%       \includegraphics[width=\textwidth]{figures/comparison/scene0024_sofa/our_stack.png}
%       \caption{Ours}
%       \end{subfigure}
      
%     \caption{Scannet scenes}
%     \label{fig:quads}
% \end{figure*}

%We use the RGB views of a part of the trajectory (TODO frames) for learning/fine-tuning, and the remaining RGB views (TODO frames) for the evaluation of different methods. We use the peak signal-noise ration (PSNR) and structured self-similarity (SSIM) measures to estimate the accuracy of the rendering for different methods on hold-out views.
\subsubsection{Comparison with state-of-the-art.} We compare our method to several neural rendering approaches on the evaluation scenes. Most of these approaches have a rendering network similar to our method, which takes an intermediate representation and then is trained to output the final RGB image. Unless stated otherwise, we use the network described in Section~\ref{sect:methods}. It is lightweight with 1.96M parameters and allows us to render real-time, taking 62ms on GeForce RTX 2080 Ti to render a FullHD image. For all the approaches we use the same train time augmentations, particularly random 512x512 crops and 2x zoom-in and zoom-out.

% \begin{itemize}
%     \item \textbf{Ours-adapted.} This is a variant of our system, where the rendering network and the descriptor space are pretrained on the 52 ScanNet scenes. Then we learn the neural descriptors and fine-tune (adapt) the rendering network on the fitting part of the evaluation scene. Such fine-tuning converges after 30 epochs (8 minutes to 1.5 hours on 4x NVIDIA Tesla V-100 depending on the size of the scene).
    
%     \item \textbf{Ours-universal.} In this variant, we do the same as above. However the rendering network is not fine-tuned for the evaluation scheme and is kept fixed, while the neural descriptors of the points are trained. Keeping the rendering network ``universal'', i.e.\ unadapted to a specific scene may be more practical in many scenarios. Such learning converges after 20 epochs (5 minutes to 1 hour on 4x NVIDIA Tesla V-100 depending on the size of the scene).
    
%     \item \textbf{Ours-Scene.} In this variant, we do not pretrain the rendering network, and instead learn it on the evaluation scene (its fitting part) only, alongside the point descriptors. Naturally, such approach is more prone to overfitting. Such learning converges after 50 epochs (12 minutes to 2.5 hours on 4x NVIDIA Tesla V-100 depending on the size of the scene).
    
%     \item \textbf{Mesh+Texture.} In this baseline, given the mesh of the scene obtained with BundleFusion or Metashape, we learn the texture via backpropagation of the same loss as used in our method through the texture mapping process onto the texture map. This results in a ``classical'' scene representation of the textured mesh.
    
%     \item \textbf{Mesh+RenderNet.} In this variant (similar to e.g.\ LookinGood~\cite{Martin18}), we additionally learn the rendering network that maps the rasterizations of the textured mesh into the final RGB images. The rendering network has the same architecture as ours (except that the input has three channels), and the learning uses the same loss as ours.
    
%     \item \textbf{Direct RenderNet.} In this variant, we evaluate an ablation of our point-based system without neural descriptors. Here, we learn the rendering network that maps the point cloud rasterized in the same way as in our method. However, instead of neural descriptors, we use the color of the point (taken from the original RGBD scan/RGB image), the 3D coordinate of the point, and the viewpoint direction $v_i$ as a 9D pseudocolor. The rendering network is then trained with the same loss as ours. The rendering network is also pretrained on the set of 52 scenes.
    
%     \item \textbf{Direct RenderNet (slow).} We observed that the Direct RenderNet variant described above benefits considerably from higher-capacity and slower rendering network. We therefore evaluated the variant with the rendering network with doubled number of channels in all intermediate layers (resulting in ~4x params, ~4x FLOPs).
    
%     %We use two variants of network for DirectTranslation. The first with the same number of parameters as ours, the second twice large than ours. The reason behind increasing capacity of the network is to allow the network to better fit a scene. It makes comparison with our method more fair since our method learns point cloud features which are separate from the rendering network.
% \end{itemize}

%\subsubsection{ScanNet}

The following methods were compared:
\begin{itemize}
    \item \textbf{Ours.} During learning, we both optimize the neural descriptors and fine-tune the rendering network on the fine-tuning part. 
    
    \item \textbf{Pix2Pix.} In this variant, we evaluate an ablation of our point-based system without neural descriptors. Here, we learn the rendering network that maps the point cloud rasterized in the same way as in our method. However, instead of neural descriptors, we use the color of the point (taken from the original RGBD scan/RGB image). The rendering network is then trained with the same loss as ours.
    
    \item \textbf{Pix2Pix (slow).} We observed that our method features neural descriptors which increases the number of parameters to be learned. For the sake of fair comparison, we therefore evaluated the variant of Pix2Pix with the rendering network with doubled number of channels in all intermediate layers (resulting in $\sim$4x parameters and FLOPs).
    
    \item \textbf{Neural Rerendering in the Wild.} Following~\cite{Meshry19}, we have augmented the input of the Pix2Pix method with the segmentation labels (one-hot format) and depth values. We have not used the appearance modeling from \cite{Meshry19}, since lightning was consistent within each dataset.
    
    \item \textbf{Neural Rerendering in the Wild (slow).} Same as previous, but twice larger number of channels in the rendering network. Due to the need to have meaningful segmentation labels, we have considered this and the previous methods only for ScanNet comparisons, where such labels are provided with the dataset.
    
    \item \textbf{Mesh+Texture.} In this baseline, given the mesh of the scene obtained with either BundleFusion or Metashape (depending on the dataset used), we learn the texture via backpropagation of the same loss as used in our method through the texture mapping process onto the texture map. This results in a ``classical'' scene representation of the textured mesh.
    
    \item \textbf{Deferred Neural Rendering (DNR).} We implemented the mesh-based approach described in ~\cite{Thies19}. As suggested, we use hierarchical neural textures with five scales (maximum $2048{\times}2048$) each having eight channels (same as the descriptor size $M$ in our method). The rendering network is then trained with the same loss as ours. Generally, this method can be seen as the analog of our method with point-based geometric proxy replaced with mesh-based proxy. %We employ texture $L_2$-regularization as in ~\cite{Thies19} with weights 8, 4, 2, 0 for the highest, medium, low and lowest textures accordingly.
\end{itemize}

%\textit{ScanNet comparison.} In all compared approaches, whenever it is possible, the rendering network is pretraned on the 100 ScanNet scenes.

% We have also invested a significant effort into adapting the surface lightfields approach~\cite{Chen18} to our data. We, however, seldom observe any improvement over the Mesh+Texture variant, and on average the results on hold-out data was worse. Apparently, surface light field estimation is not suitable for the cases when the mesh geometry is coarse.

%\subsubsection{People}
%\label{subsubsection:People}

%We additionally compare approaches on our dataset of 41 people. The rendering network, whenever it is possible, is pretrained on 102 people scenes selected for training. For all methods, metrics were calculated for images with the background masked white.

%\subsubsection{Additional scenes}
We compare the methods on ScanNet (two scenes following pretraining on 100 other scenes), on People (two people following pretraining on 102 scenes of 38 other people), as well as on 'Owl' and 'Plant' scenes (following the pretraining on People). The quantitative results of the comparison are shown in Table~\ref{tab:comparison_with_others}. All comparisons are measured on the holdout parts, for which we compare the obtained and the ground truth RGB images. We stress that we keep the holdout viewpoints sufficiently dissimilar from the viewpoints of images used for fine-tuning. For all experiments \textit{nearest train view} is defined as follows. Given a novel view, we sort train views by angle deviation from the novel view, then leave top 5\% closest by angle and pick the view closest by distance. Angle proximity is more critical since we use zoom augmentation in training which compensate distance dissimilarity. % (\fig{TODO} shows typical distance, the supplementary video shows generalization to more extreme viewpoints).

%We evaluate our method on two additional scenes -- \textbf{'Plant'} and \textbf{'Owl'} --- with respect to the same loss functions. For the \textbf{'Plant'}, we fine-tune the network after taking a checkpoint from training on \textbf{People}, and for the \textbf{'Owl'}, a checkpoint from training on \textbf{Scannet} was selected. All frames of both scenes were segmented manually via tools from Adobe Photoshop CC software package in advance, and all metrics were calculated only for the foreground pixels selected.

%Additionally, we compared with the voxel-based rendering method Neural Volumes described in~\cite{Lombardi19}. PyTorch implementation provided by the authors was used. Despite the potential expressiveness of results provided by this method, it was impossible to work with it at high resolution due to the GPU memory constraints. Images of all investigated scenes were preliminary downsampled to 768 resolution (on the long side) for this method, and it was trained on each particular scene, as per its design. Camera intrinsics and extrinsics for each frame were calculated by Agisoft Metashape, and thus may be not as accurate as ones provided by any preliminary extrinsics estimation procedure (e.g. checkerboard), however, this error is inevitable in a real scenario with one camera moving Table 3: Dependency of the loss function values on the number of Scannet scenes used toalong a random trajectory. TODO CHECK RESOLUTION.



We report the value of the loss on the holdout part (\textit{VGG}) as well as two common metrics (Learned Perceptial Similarity -- \textit{LPIPS}~\cite{Zhang18} and Frechet Inception Distance -- \textit{FID}~\cite{Heusel17}). We also show qualitative comparisons on the holdout set frames in Figures~\ref{fig:studio-holdout}--\ref{fig:plant-holdout}, where we also show the point cloud, and renderings from completely different viewpoints in Figures~\ref{fig:far_views_people}--\ref{fig:far_views_things_scannet}. Further comparisons can be found in \textbf{Supplementary video}. 

Generally, both the quantitative and the qualitative comparison reveals the advantage of using \textit{learnable neural descriptors for neural rendering}. Indeed, with the only exception (VGG metric on Person 1), Deferred Neural Rendering and Neural Point-Based Graphics, which use such learnable descriptors, outperform other methods, sometimes by a rather big margin. 

The relative performance of the two methods that use learnable neural descriptors (ours and DNR) varies across metrics and scenes. Generally, our method performs better on scenes and parts of the scene, where meshing is problematic due to e.g.~thin objects such as 'Studio' (Fig.~\ref{fig:studio-holdout}) and 'Plant' (Fig.~\ref{fig:plant-holdout}) scenes. Conversely, DNR has advantage whenever a good mesh can be reconstructed. %, such as 'Owl' scene (\fig{plant_owl}-bottom).

In support of this observations, user study via Yandex.Toloka web platform was conducted for ScanNet 'Studio' scene and 'Plant' scene. As for 'Studio', we took 300 half image size crops in total uniformly sampled from all holdout images. Labelers were asked to evaluate which picture is closer to a given ground truth crop --- produced by our method or the one produced by DNR. As for 'Plant', 100 random crops of $\frac{1}{6.5}$ original image size were selected. Users have preferred Ours vs. Deferred in \textbf{49.7\% vs. 50.3\%} cases for 'Studio' and in \textbf{69\% vs. 31\%} for 'Plant'. As before, our method performs significantly better when meshing procedure fails in the presence of thin objects and yields results visually similar to DNR when the mesh artefacts are relatively rare.

%\textbf{using the point cloud as the geometric proxy}. Thus, Mesh+\linebreak Texture and Deferred Neural Rendering perform worse than all methods that use the point clouds. The exception is the \textbf{'Owl'} scene, where the meshing procedure was successful at generating a reasonably good mesh. In all other scenes, there are parts of the scene where the meshing process (BundleFusion or Metashape) has failed, leading to gross mistakes in the renderings. The qualitative comparison reveals such failures that are particularly notorious on thin objects (such as the details of the bicycle in \fig{studio} or the leaves of the plant in \fig{plant_owl}).

%We also observe that our system based on neural descriptors of the point generally outperforms the direct RenderNet ablation, which does not have such descriptors. We also note that our holdout frames are not too far from the fitting set, and we observe that qualitatively the difference between methods becomes larger when camera is moved further from the fitting set cameras. The effect of this can be observed in \textbf{supplementary video}. Generally, the quality of single frames for such camera positions is considerably better for our method than for the Direct baseline (which suffers from blurriness and loss of details). % At the same time, admittedly, this strong improvement in the quality of individual frames comes at the price of increased temporal flickering. % is it true? maybe we can avoid flickering with supersampling, at the same time maintaining high quality of the results?

\begin{figure*}[!h]
\centering
    %\begin{subfigure}
        \begin{overpic}[trim={0 5cm 0 0}, clip, width=.45\textwidth]{figures/ours_various/olya_pretrain_people_ours_0_infer_ours.jpg}
            \put(-5,-5){\includegraphics[width=.15\textwidth]{figures/ours_various/olya_pretrain_people_ours_0_infer_nearest_train.jpg}}
        \end{overpic}
        \begin{overpic}[trim={0 5cm 0 0}, clip, width=.45\textwidth]{figures/ours_various/sasha_pretrain_people_ours_0_infer_ours.jpg}
            \put(-5,-5){\includegraphics[width=.15\textwidth]{figures/ours_various/sasha_pretrain_people_ours_0_infer_nearest_train.jpg}}
        \end{overpic}
    %\end{subfigure}
    % \rotatebox[origin=c]{90}{Ours}
    % \begin{subfigure}{0.35\linewidth}
    % \includegraphics[trim={0 0 0 0}, clip,width=\textwidth]{figures/ours_various/olya_pretrain_people_ours_0_infer_ours.png}
    % \end{subfigure}
    % \begin{subfigure}{0.35\linewidth}
    % \includegraphics[trim={0 0 0 0}, clip,width=\textwidth]{figures/ours_various/sasha_pretrain_people_ours_0_infer_ours.png}
    % \end{subfigure}
    % \hfill
    
    % \hfill
    % \rotatebox[origin=c]{90}{Nearest train view}
    % \begin{subfigure}[c]{0.15\linewidth}
    % \includegraphics[trim={0 0 0 0}, clip,width=\textwidth]{figures/ours_various/olya_pretrain_people_ours_0_infer_nearest_train.JPG}
    % \end{subfigure}
    % \hfill
    % \begin{subfigure}{0.15\linewidth}
    % \includegraphics[trim={0 0 0 0}, clip,width=\textwidth]{figures/ours_various/sasha_pretrain_people_ours_0_infer_nearest_train.png}
    %\end{subfigure}
    % \hfill
    
    % \rotatebox[origin=c]{90}{Ours}
    % \begin{subfigure}{0.35\linewidth}
    % \includegraphics[trim={0 0 0 0}, clip,width=\textwidth]{figures/ours_various/owl2_pretrain_people_ours_0_infer_ours.png}
    % \end{subfigure}
    % \begin{subfigure}{0.35\linewidth}
    % \includegraphics[trim={0 0 0 0}, clip,width=\textwidth]{figures/ours_various/plant_pretrain_people_ours_0_infer_ours.png}
    % \end{subfigure}
    % \hfillnovel
    
    % \hfill
    % \rotatebox[origin=c]{90}{Nearest train view}
    % \begin{subfigure}{0.15\linewidth}
    % \includegraphics[trim={0 10.3cm 0 10.3cm}, clip,width=\textwidth]{figures/ours_various/owl2_pretrain_people_ours_0_infer_nearest_train.jpg}
    % \end{subfigure}
    % \hfill
    % \begin{subfigure}{0.15\linewidth}
    % \includegraphics[trim={0 10.3cm 0 10.3cm}, clip,width=\textwidth]{figures/ours_various/plant_pretrain_people_ours_0_infer_nearest_train.png}
    % \end{subfigure}
    % \hfill
    \vspace{0.4cm}
    \caption{Novel views of \textbf{People} generated by our method (\textit{large picture}: our rendered result, \textit{small overlaid picture}: nearest view from the fitting part). Both people are from the holdout part (excluded from pretraining).}
    \label{fig:far_views_people}
\end{figure*}
% \begin{figure*}[!h]
% \centering
%     %\begin{subfigure}
%         \begin{overpic}[width=.35\textwidth]{figures/ours_various/owl2_pretrain_people_ours_0_infer_ours.png}
%             \put(0, 0){\includegraphics[trim={22cm 30cm 13cm 30cm}, clip, width=.1\textwidth]{figures/ours_various/owl2_pretrain_people_ours_0_infer_nearest_train.JPG}}
%         \end{overpic}
%         \begin{overpic}[width=.35\textwidth]{figures/ours_various/plant_pretrain_people_ours_0_infer_ours.png}
%             \put(0, 0){\includegraphics[trim={13cm 30cm 23cm 30cm}, clip, width=.1\textwidth]{figures/ours_various/plant_pretrain_people_ours_0_infer_nearest_train.png}}
%         \end{overpic}
%     \vspace{0.2cm}
%     \caption{Novel views of \textbf{Plant} and \textbf{Owl} generated by our method (same format as in Fig.~\ref{fig:far_views_people}).}
%     \label{fig:far_views_things}
% \end{figure*}
% \begin{figure*}[!h]
% \centering
%     \rotatebox[origin=c]{90}{Ours}
%     \begin{subfigure}{0.35\linewidth}
%     \includegraphics[trim={0 0 0 0}, clip,width=\textwidth]{figures/ours_various/745_ours.png}
%     \end{subfigure}
%     \begin{subfigure}{0.35\linewidth}
%     \includegraphics[trim={0 0 0 0}, clip,width=\textwidth]{figures/ours_various/2210_ours.png}
%     \end{subfigure}
%     \hfill
    
%     \rotatebox[origin=c]{90}{Nearest train view}
%     \begin{subfigure}{0.35\linewidth}
%     \includegraphics[trim={0 0 0 0}, clip,width=\textwidth]{figures/ours_various/745_nearest_train.jpg}
%     \end{subfigure}
%     \begin{subfigure}{0.35\linewidth}
%     \includegraphics[trim={0 0 0 0}, clip,width=\textwidth]{figures/ours_various/2210_nearest_train.jpg}
%     \end{subfigure}second row:
%     \caption{Various results obtained by our method. Images in the second row correspond to the nearest train view for each of the images in the first row.}
%     \label{fig:plant_owl}
% \end{figure*}
\begin{figure*}[!h]
\centering
    \begin{subfigure}[b]{0.48\linewidth}
        \centering
        \begin{overpic}[width=.49\textwidth]{figures/ours_various/owl2_pretrain_people_ours_0_infer_ours.jpg}
            \put(0, 0){\includegraphics[trim={11cm 16.5cm 6.5cm 22.5cm}, clip, width=.2\textwidth]{figures/ours_various/owl2_pretrain_people_ours_0_infer_nearest_train.jpg}}
            %\caption{\textbf{Owl}}
        \end{overpic}
        \begin{overpic}[width=.49\textwidth]{figures/ours_various/plant_pretrain_people_ours_0_infer_ours.jpg}
            \put(0, 0){\includegraphics[trim={6.5cm 16.5cm 11.5cm 22.5cm}, clip, width=.2\textwidth]{figures/ours_various/plant_pretrain_people_ours_0_infer_nearest_train.jpg}}
            %\caption{\textbf{Plant}}
        \end{overpic}
        \captionsetup{width=.9\linewidth}
        \caption{\textbf{'Owl'} and \textbf{'Plant'}. \textit{Large picture:} render from a novel point, \textit{small overlaid picture:} nearest train view}
    \end{subfigure}
    \begin{subfigure}[b]{0.48\linewidth}
        % horizontal alignment:
        \centering
        \begin{subfigure}{0.48\linewidth}
            \includegraphics[trim={0 0 0 0}, clip,width=\textwidth]{figures/ours_various/745_ours.jpg}
        \end{subfigure}
        \begin{subfigure}{0.48\linewidth}
            \includegraphics[trim={0 0 0 0}, clip,width=\textwidth]{figures/ours_various/745_nearest_train.jpg}
        \end{subfigure}
        %\hfill
        
        \centering
        \begin{subfigure}{0.48\linewidth}
        \includegraphics[trim={0 0 0 0}, clip,width=\textwidth]{figures/ours_various/2210_ours.jpg}
        \caption*{Ours}
        \end{subfigure}
        \begin{subfigure}{0.48\linewidth}
        \includegraphics[trim={0 0 0 0}, clip,width=\textwidth]{figures/ours_various/2210_nearest_train.jpg}
        \caption*{Nearest train view}
        \end{subfigure}
        
        % vertical alignment:
        % \rotatebox[origin=c]{90}{\scriptsize Ours}
        % \begin{subfigure}{0.45\linewidth}
        %     \includegraphics[trim={0 0 0 0}, clip,width=\textwidth]{figures/ours_various/745_ours.jpg}
        % \end{subfigure}
        % \begin{subfigure}{0.45\linewidth}
        %     \includegraphics[trim={0 0 0 0}, clip,width=\textwidth]{figures/ours_various/2210_ours.jpg}
        % \end{subfigure}
        % %\hfill
        
        % \centering
        % \rotatebox[origin=c]{90}{\scriptsize Nearest train view}
        % \begin{subfigure}{0.45\linewidth}
        % \includegraphics[trim={0 0 0 0}, clip,width=\textwidth]{figures/ours_various/745_nearest_train.jpg}
        % \end{subfigure}
        % \begin{subfigure}{0.45\linewidth}
        % \includegraphics[trim={0 0 0 0}, clip,width=\textwidth]{figures/ours_various/2210_nearest_train.jpg}
        % \end{subfigure}
        \captionsetup[subfigure]{position=b, width=.9\linewidth}
        \caption{\textbf{'Studio'}. \textit{First row:} render from a novel point, \textit{second row:} nearest train view}
    \end{subfigure}
    \caption{Various results obtained by our method. For each of the scenes, we show the view from the nearest camera from the fine-tuning part (\textit{nearest train view}).}
    \label{fig:far_views_things_scannet}
\end{figure*}


%\subsection{Ablation study}

\subsubsection{Ablation study.} We also evaluate the effect of some of the design choices inside our method. First, we consider the point cloud density and the descriptor size. We take an evaluation scene from ScanNet and progressively downsample point cloud using voxel downsampling and get small, medium and large variants with 0.5, 1.5, and 10 million points respectively. For each variant of point cloud we fit descriptors with sizes $M$ equal to 4, 8 (default) and 16. \tab{desc_size} shows evaluation results. It naturally reveals the advantage of using denser point clouds, yet it also shows that the performance of our method saturates at $M=8$.

% We further investigate the effect of pretraining by considering pretraining on 200, 100 (default), 50, and 0 scenes (in the latter case, the network weights are initialized randomly before fine-tuning). Further, we consider the scenario, when the network weights are kept fixed during fine-tuning. The results in \tab{pretraining} reveal that our method is not overly sensitive to the size of pretraining dataset, while the results with fixed rendering network are noticeably worse. We note that qualitatively, we observe the advantage of having pretraining is strong, when generalizing to very different viewpoints (\fig{pretraining}).

% We have also compared extensively with the variant of the method without progressive rendering (i.e.\ where the rendering network receives the raw image only at the finest scale). To make such result competitive one needs to add splatting. After we have added square image-parallel splats with the splat size tuned to the ScanNet dataset, we have observed that this variant performed comparably with our default method (better in VGG and LPIPS metrics, worse in FID metric). However, using the same splat size for the people dataset resulted in a uniformly worse performance across all metrics. 

\begin{table}[!h]
    \centering
    \caption{Dependency of the loss function values on the descriptor size and the point cloud size. Comparison is made for the 'Studio' scene of Scannet.}
    \vspace{0.1cm}
    \begin{tabular}{l|c|c|c|c|c|c}
                                     & \multicolumn{2}{c|}{\,Descriptor size 4\,}                                             & \multicolumn{2}{c|}{\,Descriptor size 8\,}                                             & \multicolumn{2}{c}{\,Descriptor size 16\,}                                            \\
    Point Cloud size                 & VGG $\downarrow$    & LPIPS $\downarrow$& VGG  $\downarrow$    & LPIPS  $\downarrow$ & VGG $\downarrow$    & LPIPS $\downarrow$ \\ \hline
    \textit{small}  & 635.74                           & 0.543                           & 632.39                           & 0.505                           & 622.06                           & 0.508                           \\
    \textit{medium} & 622.05                           & 0.506                           & 616.49                           & 0.486                           & 614.90                           & 0.500                           \\
    \textit{large}  & \textbf{610.76} & \textbf{0.509}                           & \textbf{\underline{609.11}} & \textbf{\underline{0.485}}                           & \textbf{611.38} & \textbf{0.488}                         
    \end{tabular}
    \label{tab:desc_size}
\end{table}


% SCENE EDITING: PLANT ONLY
\begin{figure*}[!h]
    \centering
    \captionsetup[subfigure]{labelformat=empty, justification=centering}
      \begin{subfigure}{0.31\linewidth}
      \includegraphics[trim={0 22.5cm 7.5cm 0}, clip,width=\linewidth]{figures/scene_editing/egor_aloe_2/egor_pretrain_people_ours_0_infer.jpg}
      \caption{original scene\\ \,}
      \end{subfigure}
      \begin{subfigure}{0.31\linewidth}
      \includegraphics[trim={0 22.5cm 7.5cm 0}, clip, width=\linewidth]{figures/scene_editing/egor_aloe_2/egor_aloe_pc_close_p2.jpg}
      \caption{Person 2 + Plant: point cloud composition}
      \end{subfigure}
    %   \begin{subfigure}{0.19\linewidth}
    %   \includegraphics[trim={0 45cm 15cm 0}, clip, width=\linewidth]{figures/scene_editing/egor_aloe_2/egor_aloe_pix2pix_0_infer.jpg}
    %   \caption{Pix2Pix}
    %   \end{subfigure}
      \begin{subfigure}{0.31\linewidth}
      \includegraphics[trim={0 22.5cm 7.5cm 0}, clip, width=\linewidth]{figures/scene_editing/egor_aloe_2/egor_aloe_ours_0_infer.jpg}
      \caption{Person 2 + Plant: ours}
      \end{subfigure}
    \caption{A novel view for the composed scenes. A point cloud from 'Plant’ scene was translated and rotated slightly to be placed on the left hand of the 'Person 2'. The world scale of objects was kept unchanged.}
    \label{fig:scene_editing}
\end{figure*}

% % SCENE EDITING: OWL+PLANT ONE ROW
% \begin{figure*}[!h]
%     \centering
%     \captionsetup[subfigure]{labelformat=empty, justification=centering}
%       \begin{subfigure}{0.19\linewidth}
%       \includegraphics[trim={0 5cm 0 20cm}, clip,width=\linewidth]{figures/scene_editing/1/egor_pretrain_scannet_ours_frozen_0_infer.jpg}
%       \caption{original scene\\ \,}
%       \end{subfigure}
%       \begin{subfigure}{0.19\linewidth}
%       \includegraphics[trim={0 5cm 0 20cm}, clip, width=\linewidth]{figures/scene_editing/1/egor_owl_ours_frozen_0_colors_p2.jpg}
%       \caption{Person 2 + Owl: point cloud}
%       \end{subfigure}
%     %   \begin{subfigure}{0.19\linewidth}
%     %   \includegraphics[trim={0 5cm 0 20cm}, clip, width=\linewidth]{figures/scene_editing/1/egor_owl_pix2pix_heavy_0_infer.jpg}
%     % %   \caption{Direct\\ \,}
%     %   \end{subfigure}
%       \begin{subfigure}{0.19\linewidth}
%       \includegraphics[trim={0 5cm 0 20cm}, clip, width=\linewidth]{figures/scene_editing/1/egor_owl_ours_frozen_0_infer.jpg}
%       \caption{Person 2 + Owl: ours}
%       \end{subfigure}
%     %   \begin{subfigure}{0.19\linewidth}
%     %   \includegraphics[trim={0 45cm 15cm 0}, clip,width=\linewidth]{figures/scene_editing/egor_aloe_2/egor_pretrain_people_ours_0_infer.jpg}
%     %   \caption{original scene\\ \,}
%     %   \end{subfigure}
%       \begin{subfigure}{0.19\linewidth}
%       \includegraphics[trim={0 45cm 15cm 0}, clip, width=\linewidth]{figures/scene_editing/egor_aloe_2/egor_aloe_pc_close_p2.jpg}
%       \caption{Person 2 + Plant: point cloud composition}
%       \end{subfigure}
%     %   \begin{subfigure}{0.19\linewidth}
%     %   \includegraphics[trim={0 45cm 15cm 0}, clip, width=\linewidth]{figures/scene_editing/egor_aloe_2/egor_aloe_pix2pix_0_infer.jpg}
%     %   \caption{Pix2Pix}
%     %   \end{subfigure}
%       \begin{subfigure}{0.19\linewidth}
%       \includegraphics[trim={0 45cm 15cm 0}, clip, width=\linewidth]{figures/scene_editing/egor_aloe_2/egor_aloe_ours_0_infer.jpg}
%       \caption{Person 2 + Plant: ours}
%       \end{subfigure}
%     \caption{A novel view for the composed scenes. An 'Owl' and 'Plant’ scenes were translated and rotated slightly to be placed on the left hand of the 'Person 2'. The world scale of objects was kept unchanged.} 
%     \label{fig:scene_editing}
% \end{figure*}

% % SCENE EDITING: OWL+PLANT GRID
% \begin{figure*}[!h]
%     \centering
%     \captionsetup[subfigure]{labelformat=empty, justification=centering}
%     \begin{subfigure}{.45\textwidth}
%         \centering
%         \begin{subfigure}{.3\textwidth}
%             \begin{subfigure}{.95\textwidth}
%                 \includegraphics[trim={0 5cm 0 20cm}, clip,width=\linewidth]{figures/scene_editing/1/egor_pretrain_scannet_ours_frozen_0_infer.jpg}
%                 \caption{\tiny original scene\\ \,}
%             \end{subfigure}
            
%             \begin{subfigure}{.95\linewidth}
%                 \includegraphics[trim={0 5cm 0 20cm}, clip, width=\linewidth]{figures/scene_editing/1/egor_owl_ours_frozen_0_colors_p2.jpg}
%                 \caption{\tiny Person 2 + Owl: point cloud}
%             \end{subfigure}
%         \end{subfigure}
%         \begin{subfigure}[c]{.68\linewidth}
%             \includegraphics[trim={0 5cm 0 20cm}, clip, width=\linewidth]{figures/scene_editing/1/egor_owl_ours_frozen_0_infer.jpg}
%             \caption{Person 2 + Owl: ours\\ \,}
%         \end{subfigure}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{.45\textwidth}
%         \centering
%         \begin{subfigure}{.3\textwidth}
%             \begin{subfigure}{.95\textwidth}
%                 \includegraphics[trim={0 45cm 15cm 0}, clip,width=\linewidth]{figures/scene_editing/egor_aloe_2/egor_pretrain_people_ours_0_infer.jpg}
%                 \caption{\tiny original scene\\ \,}
%             \end{subfigure}
            
%             \begin{subfigure}{.95\linewidth}
%                 \includegraphics[trim={0 45cm 15cm 0}, clip, width=\linewidth]{figures/scene_editing/egor_aloe_2/egor_aloe_pc_close_p2.jpg}
%                 \caption{\tiny Person 2 + Plant: point cloud}
%             \end{subfigure}
%         \end{subfigure}
%         \begin{subfigure}[c]{.68\linewidth}
%             \includegraphics[trim={0 45cm 15cm 0}, clip, width=\linewidth]{figures/scene_editing/egor_aloe_2/egor_aloe_ours_0_infer.jpg}
%             \caption{Person 2 + Plant: ours\\ \,}
%         \end{subfigure}
%     \end{subfigure}
% \end{figure*}

% pretrain tables [temporarily commented]:
% \begin{table}[!h]
%     \centering
%     \caption{Dependency of the loss function values on the number of Scannet scenes used to pretrain the rendering network. Comparison is made for the 'Studio' scene of Scannet. \textit{None} refers to no pretraining.}
%     \vspace{0.1cm}
%     \begin{tabular}{l|c|c|c}
%     Pretraining                      & VGG $\downarrow$ & LPIPS $\downarrow$ & FID $\downarrow$ \\ \hline
%     None                             & 607.63           & \textbf{0.468}     & 79.75            \\
%     On 50 scenes                     & \textbf{594.79}  & 0.471              & 78.56            \\
%     \textit{On 100 scenes (default)} & 595.24           & 0.472              & \textbf{76.72}   \\
%     On 200 scenes                    & 595.06           & 0.472              & 76.91     \\ \hline
%     On 100 scenes; no fine-tuning\,  & 603.18           & 0.485              & 81.97    
%     \end{tabular}
%     \label{tab:pretraining}
% \end{table}

% \begin{figure*}[!h]
%     \centering
%     \captionsetup[subfigure]{justification=centering,labelformat=empty}
%       \begin{subfigure}{0.30\linewidth}
%       \includegraphics[trim={0 0 0 0}, clip,width=\linewidth]{figures/ablation_pretrain/ts_1_ts_1_scratch_stack.jpg}
%       %\caption{No pretraining\\ \,}
%       \end{subfigure}
%       \begin{subfigure}{0.30\linewidth}
%       \includegraphics[trim={0 0 0 0}, clip,width=\linewidth]{figures/ablation_pretrain/ts_1_ts_1_pretrain_stack.jpg}
%       %\caption{Pretrained on 100 Scannet scenes}
%       \end{subfigure}
%       \begin{subfigure}{0.30\linewidth}
%       \includegraphics[trim={0 0 0 0}, clip,width=\linewidth]{figures/ablation_pretrain/ts_1_ts_1_nearest_train_stack.jpg}
%       %\caption{Nearest train view\\ \,}
%       \end{subfigure}
%       \hfill
%       \begin{subfigure}{0.30\linewidth}
%       \includegraphics[trim={0 0 0 0}, clip,width=\linewidth]{figures/ablation_pretrain/ts_2_ts_2_scratch_stack.jpg}
%       \caption{No pretraining\\ \,}
%       \end{subfigure}
%       \begin{subfigure}{0.30\linewidth}
%       \includegraphics[trim={0 0 0 0}, clip,width=\linewidth]{figures/ablation_pretrain/ts_2_ts_2_pretrain_stack.jpg}
%       \caption{Pretrained on 100 scenes}
%       \end{subfigure}
%       \begin{subfigure}{0.30\linewidth}
%       \includegraphics[trim={0 0 0 0}, clip,width=\linewidth]{figures/ablation_pretrain/ts_2_ts_2_nearest_train_stack.jpg}
%       \caption{Nearest train view\\ \,}
%       \end{subfigure}
%     \caption{Comparison of the renderings of 'LivingRoom' Scannet scene from viewpoints located far from the shooting trajectory (small cropped areas were selected). Here we assess whether pretraining helps the network to generalize to new viewpoints.} 
%     \label{fig:pretraining}
% \end{figure*}

% \subsubsection{Pretraining}

% In this section we show the advantage of pretraining the rendering network.

% \begin{itemize}
%     \item Fit network from scratch
%     \item Freeze pretrained network
%     \item Finetune pretrained network
%     \item Fit plant descriptors for network pretrainPlanted on people
% \end{itemize}

% \subsubsection{Rendering method}

% In this section we show the advantage of progressive rendering over square splatting both qualitatively and quantitatively. We evaluate these methods on a ScanNet scene using pretrained rendering network.

% \vspace{-0.3cm}
% \begin{figure}
%   \centering
%   \includegraphics[width=0.3\textwidth]{figures/scene_editing/egor_owl2.jpg}%\hspace{0.3cm}
%   \label{fig:edt_owl}
% \end{figure}

% Usage of a shared rendering network allows to compose new scenes by combining proxy point clouds and corresponding learned descriptors. Assuming the objects have roughly the same 3d orientation one could apply basic transformations (translation, scaling and slight rotation) to initial point clouds if needed to align objects in the world space. The composed scene is further obtained by combining respectively XYZ points and learned descriptors for all objects into a new point cloud with corresponding descriptors.

\subsubsection{Scene editing.} To conclude, we show a qualitative example of creating a composite of two separately captured scenes (Fig.~\ref{fig:scene_editing}). To create it, we took the 'Person 2' and the 'Plant' datasets and fitted descriptors for them while keeping the rendering network, pretrained on People, frozen. We then align the two point clouds with learned descriptors by a manually-chosen rigid transform and created the rendering.

\subsubsection{Anti-aliasing.} We have found that in the presence of camera misregistrations in the fitting set (such as ScanNet scenes), our method tends to produce flickering artefacts during camera motion (as opposed to \cite{Thies19} that tends to produce blurry outputs in these cases). At least part of this flickering can be attributed to rounding of point projections to the nearest integer position during rendering. It is possible to generate each of the raw images at higher resolution (e.g.\ 2$\times$ or 4$\times$ higher), and then downsample it to the target resolution using bilinear interpolation resulting in smoother raw images. This results in less flickering with a cost of barely noticeable blur (see \textbf{supplementary video}). Note that the increase in time complexity from such anti-aliasing is insignificant, since it does not affect the resolution at which neural rendering is performed.



% In this section we show that, given a trained rendering network, one can render multiple 3D objects as a single scene. The idea is the following. By taking such a network, one can learn neural descriptors separately for multiple point clouds, at the same time keeping the network frozen. This way, the composition can be obtained by spatial alignment of individual point clouds into one.

% The scenes 'Person 2’ and ‘Plant’ have been introduced before in Section~\ref{subsect:datasets}. Additionally, we took another sequence of photos of \textbf{'Owl'} by a mirrorless camera that could better capture details and reflections of this model. We will refer to this data as \textbf{'Owl*'}. We demonstrate the scene editing pipeline on two combinations: \textbf{'Person 2' + 'Owl*'} and \textbf{'Person 2' + 'Plant'}. To produce the results depicted in Fig.~\ref{fig:scene_editing}, we first take a rendering network trained on \textbf{Scannet}, and then independently learn neural descriptors for each of two scenes to be combined. During the optimization of descriptors, the rendering network remains frozen. To render the resulting merged scene, we "put" an object (\textbf{'Owl*'} or \textbf{'Plant'}) on top of \textbf{'Person 2'}s hand by a translation and rotation of the object. 

% For this experiment, the ground truth images of 'Person 2' were automatically segmented by "Select subject" tool from Adobe Photoshop CC software package before fine-tuning to alleviate all potential errors of CNN-based segmentation used for training. Segmentation for the sequences \textbf{'Owl*'} and \textbf{‘Plant’} was obtained in a semi-automatic manner using Adobe Photoshop CC, and the point clouds for this experiment were reconstructed with background masked.    % to be reduced


% ig{comparison1} (for ScanNet scenes) and in \fig{comparison2} (for RGB scenes). 
% The following may be observed from the comparisons.


% TODO The variants of our approach outperform other methods considerably. The comparison in \fig{bicycle} highlights the particularly large advantage of our approach over the mesh-based baselines for the parts of the scene that are poorly captured by the mesh (thin parts of a bicycle, where the resolution of the volumetric grid inside BundleFusion and/or the accuracy of registration precluded accurate reconstruction).

% Importantly, the results also reveal that our approach benefits from preliminary training on the corpus of scenes and that such training allows it to generalize better to new views.

% Minor difference between DirectTranslation (heavy) and our method is due to close similarity between train and hold-out sets. It becomes apparent when rendering scenes far from the camera trajectory (\fig{quads}). DirectTranslation renderings are more blurry in comparison to ours.

% \subsection{Results on RGB datasets}

% In addition to the RGBD data, we test our approach on static scenes imaged using RGB videos taken be a modern smartphone (Samsung Galaxy S10). We use the commercial off-the-shelf software package~\cite{AgiSoft} to obtain the registration, the point cloud as well as the reconstructed mesh with texture. We then test our approach as well as the baselines (\tab{comparison}). The results are TODO.


% \subsection{Results on synthetic data}

% \begin{figure*}
%     \centering
%     %\includegraphics{}
%     \begin{tabular}{cccc}
%     %\includegraphic[width=0.24\textwidth]{figures/comparison/sphere/1195_blender.png}&
%     %\includegraphic[width=0.24\textwidth]{figures/comparison/sphere/1195_pca.png}&
%     %\includegraphic[width=0.24\textwidth]{figures/comparison/sphere/1195_color.png}&
%     %\includegraphic[width=0.24\textwidth]{figures/comparison/sphere/closest.png}\\ 
%     %\includegraphic[width=0.24\textwidth]{figures/comparison/sphere_back/0415.png}&
%     %\includegraphic[width=0.24\textwidth]{figures/comparison/sphere_back/0415_pca.png}&
%     %\includegraphic[width=0.24\textwidth]{figures/comparison/sphere_back/0415_color.png}&
%     %\includegraphic[width=0.24\textwidth]{figures/comparison/sphere_back/0406_closest.png}\\
%     Ray tracing & Point Cloud+descriptors & Our rendering (real-time) & Closest train\\
%     \end{tabular}
%     \caption{Our system can be used to speed up renderings of synthetic scenes. Here, we show renderings of the standard Blender test scene using our system (third column). The closest frame from the dataset of frames used for model fitting is shown the fourth column. While our system does not match the result of the ray tracing rendering exactly, it manages to reproduce some details in the specular reflection, and fine details in the texture, while doing so at real-time speed.}
%     \label{fig:blenderball}
% \end{figure*}


% We also show the capability of our approach to model synthetic scenes with extremely complex photometric properties (\fig{blenderball}). Here, the use of our approach may be justified as a means for accelerating rendering. Towards this end, we take the default Blender~\cite{Blender} test scene with complex lighting and highly-specular object in the center, sample a point cloud (2.5 million points) from its surface, and learn the neural descriptors and the rendering networks from 200 random views of the scene. The comparison of our renderings with the ``ground truth'' synthetic renderings obtained by ray tracing within Blender reveals very close match (\fig{blenderball}). While Blender takes about 2 minutes to render one frame of this scene on two GeForce RTX 2080 Ti (highest quality setting), our renderings are obtained at 50ms (20 frames-per-second) on one GeForce RTX 2080 Ti. We note that given the availability of a good surface mesh for this scene, mesh-based neural rendering approaches \cite{Hedman18,Chen18,Thies19} are also likely to perform well at this task.


% \subsection{Compositing}

% \begin{figure}
%     \centering
%     %\includegraphics{}
%     \caption{Insert shoe into the room and render it}
%     \label{fig:compose}
% \end{figure}

% Finally, we show that our scene representation allows editing operations such as compositing. For this, we copy the part of the point cloud from the 'Shoe' scene (enclosed by the shoe bounding box) alongside with the learned rendering network into the 'Room' scene. In this case, we kept the rendering network fixed during adaptation for both scenes, making the neural descriptors of each scene compatible with each other. As a result, the composited scene can be rendered without any post-processing (\fig{compose}).








==> intro.tex <==


\section{Introduction}
\label{sect:intro}

Creating virtual models of real scenes usually involves a lengthy pipeline of operations. Such modeling usually starts with a scanning process, where the photometric properties are captured using camera images and the raw scene geometry is captured using depth scanners or dense stereo matching. The latter process usually provides noisy and incomplete point cloud that needs to be further processed by applying certain surface reconstruction and meshing approaches. Given the mesh,  the texturing and material estimation processes determine the photometric properties of surface fragments and store them in the form of 2D parameterized maps, such as texture maps~\cite{Blinn76}, bump maps~\cite{Blinn78}, view-dependent textures~\cite{Debevec98}, surface lightfields~\cite{Wood00}. Finally, generating photorealistic views of the modeled scene involves computationally-heavy rendering process such as ray tracing and/or radiance transfer estimation.

The outlined pipeline has been developed and polished by the computer graphics researchers and practitioners for decades. Under controlled settings, this pipeline yields highly realistic results. Yet several of its stages (and, consequently, the entire pipeline) remain brittle. Multiple streams of work aim to simplify the entire pipeline by eliminating some of its stages. Thus, image-based rendering techniques~\cite{McMillan95,Seitz96,Gortler96,Levoy96} aim to obtain photorealistic views by warping the original camera images using certain (oftentimes very coarse) approximations of scene geometry. Alternatively, point-based graphics~\cite{Levoy85,Grossman98,Gross02,Kobbelt04} discards the estimation of the surface mesh and use a collection of points or unconnected disks (surfels) to model the geometry. More recently, deep rendering approaches~\cite{Isola17,Nalbach17,Chen18,Bui18,Hedman18} aim to replace physics-based rendering with a generative neural network, so that some of the mistakes of the modeling pipeline can be rectified by the rendering network.

Here, we present a system that eliminates many of the steps of the classical pipeline. It combines the ideas of image-based rendering, point-based graphics, and neural rendering into a simple approach. The approach uses the raw point-cloud as a scene geometry representation, thus eliminating the need for surface estimation and meshing. Similarly to other neural rendering approaches, it also uses a deep convolutional neural network to generate photorealistic renderings from new viewpoints. The realism of the rendering is facilitated by the estimation of latent vectors (neural descriptors) that describe both the geometric and the photometric properties of the data. These descriptors are learned directly from data, and such learning happens in coordination with the learning of the rendering network (see Fig. \ref{fig:method}).

%Unlike point-based graphics, our approach avoids the explicit estimation of surface orientation or radiance function parameters, and, instead uses backpropagation through the rendering network directly onto the raw points  in order to estimate local photometric and geometric properties. Interestingly, local appearance in our approach is described by latent vectors that are learned in parallel with the rendering network.

We show that our approach is capable of modeling and rendering scenes that are captured by hand-held RGBD cameras as well as simple RGB streams (from which point clouds are reconstructed via structure-from-motion or similar techniques). A number of comparisons are performed with ablations and competing approaches, demonstrating the capabilities, advantages, and limitations of the new method. In general, our results suggest that given the power of modern deep networks, the simplest 3D primitives (i.e.\ 3D points) might represent sufficient and most suitable geometric proxies for neural rendering in many cases.








% In this work, we propose to shortcut most of the operations in the modeling-rendering pipeline using deep convolutional \textit{scene-specific rendering networks}. A scene-specific rendering network is trained to map rasterizations of a potentially noisy and incomplete geometric proxy of a scene into novel photorealistic views of this scene. We show that such a conceptually simple pipeline can be surprisingly efficient at capturing and synthesizing new views of geometrically and photometrically complex scenes.

% Several approaches that use deep neural networks to produce the realistic renderings of a scene have been proposed \cite{HedmanPPFDB18DeepBlending,HedmanRDB16InsideOut,Sitzmann18,Chen18DeepSurfaceLightFields}. These approaches train large networks that convert certain input views or some other scene representations into new photorealistic views. The network parameters are tuned to match the appearance of the training views. The hope is then that the network generalizes to a certain set of novel views and/or new scenes distinct from the training ones. 

% The use of neural networks within these new approaches allows to eliminate some of the traditional modeling or rendering techniques that are usually needed to obtain photorealistic views. From this standpoint, these new methods follow the older generation of \textit{image-based rendering} methods of late 90s and early 2000s (\cite{seitz1996viewmorph,GortlerGSC96Lumigraph,McMillanB95Plenoptic,levoy1996light}) that used geometric warping and interpolation to achieve the same effect of eliminating certain modeling and rendering steps. Compared to classical image-based rendering, the use of neural networks learned on training views instead of geometric warping of the same views brings in extra flexibility and statistical efficiency. Furthermore, the use of new optimization objectives developed by deep learning community such as perceptual~\cite{Johnson16} and adversarial~\cite{goodfellow2014generative} losses brings in certain tolerance to registration errors. Finally, the mature state of hardware equipment and software stack for deep learning means that new systems of this kind are fast at runtime and are relatively easy to implement.

% In this work, we propose a new modeling-rendering pipeline that replaces most of the steps with a neural network. The new pipeline is applicable to both real and synthetic (i.e.\ human designed) scenes. For real scenes, our pipeline assumes the availability of a number of registered photographs or video-frames with known camera parameters. For synthetic scenes, we assume that such views have been pre-rendered using potentially complex and time-consuming photo-realistic rendering system. In the latter case, our approach allows to speed up photorealistic rendering to interactive frame rates.


% The new pipeline is organized as follows. First, a geometric proxy is estimated. When dealing with synthetic scenes, we simply take the underlying mesh as a proxy. For real scenes, a noisy and incomplete point clouds describing scene geometry are extracted from the input set of photographs using multi-view stereo matching. Note that obtaining point clouds from multi-view stereo is a well-researched area~\cite{schonberger2016structure}. Alternatively, a coarse proxy geometry may come from volumetric fusion techniques such as KinectFusion~\cite{NewcombeIHMKDKSHF11}. The main part of our pipeline is a convolutional neural network that is trained to directly map the rasterizations of the proxy geometry into a photorealistic scene view. Here, we use the original set of views as training examples for the neural network. To generate a new, previously unseen view, we simply rasterize the proxy geometry using the camera parameters of the new view, and then obtain the novel view by passing the rasterization through the neural network.

% While we are not the first to use convolutional networks for new view synthesis~\cite{wang2018vid2vid}, there are several new aspects in our system. Most importantly, the neural networks in our system are \textit{scene-specific}, therefore we name them SSNets. In other words, we fit each network to the available image data describing a particular static scene. This comes with the following benefits. First and foremost, the use of scene-specific networks allows us to use world (global) coordinates of points in the point clouds as features that we can input into the network. This is in contrast to the use of scene-agnostic networks \cite{NalbachAMSR17}, where only camera-space coordinates may be used as features. We show that the use of world-coordinates as input features allows our networks to generalize well to new views after training, while still retaining the ability to model view-dependent effects. The second advantage of scene-specific networks is that in each case, we are able to spend all network capacity entirely on the scene of interest. Our final contribution is a specific network architecture that can be used to deal with noisy and incomplete point clouds as geometric proxies. To handle such proxies, we use point cloud rasterizations at multiple resolutions and input these rasterizations at different stages of the architecture. This allows us to solve the inherent problem of point-based graphics systems that have to choose the size of the \textit{splatting disks} at individual point (which is known to be a brittle operation).

% We demonstrate the advantages of our pipeline within a set of experiments that encompass both human-designed synthesized scenes (where scene-specific rendering networks can be used to amortize render time of geometrically and photometrically-complex objects and enable real-time visualizations) as well as real scenes (where scene-specific rendering networks can be used to obtain new photorealistic views of the scene even when the estimated scene geometry is imprecise and incomplete). 

% We observe that even with limited number of input views, the approach generalizes well to new views, even in the presence of noise and large gaps in the obtained 

% In this work, we follow the same short-cutting idea. In particular, we consider deep convolutional networks that we call XYZNets. Each XYZNet is trained for a particular scene. To generate a new view of the scene, our pipeline takes the scene geometry, rasterizes the geometry to the 2D view, so that each pixel contains its world coordinates and its normal coordinates (we also use world orientation). A pretrained XYZNet then translates the rendered maps into the output RGB values.

% Notably, in the input maps, the absolute position and the normal orientation of the pixel are encoded using world coordinates. We show that XYZNets can nevertheless successfully model view-dependent effects, since the use of convolutional operations allows it to infer the view direction from the rendered views. At the same time, the focus on world coordinate representations and the lack of view-specific representations in the input allows the trained networks to achieve extra degree of generalization to new views.

==> method.tex <==
\section{Methods}
\label{sect:methods}
\def\P{\mathbf{P}}
\def\D{\mathbf{D}}
\def\C{C}
\def\Loss{\mathcal{L}}
\def\s{\mathbf{s}}
\def\Rend{\mathcal{R}}
\def\I{\mathbf{I}}

Below, we explain the details of our system. First, we explain how the rendering of a new view is performed given a point cloud with learned neural descriptors and a learned rendering network. Afterwards, we discuss the process that creates a neural model of a new scene.

\begin{figure*}
  \centering
  \includegraphics[width=1\textwidth]{figures/npbg_multiscale.pdf}
  \caption{ An overview of our system. Given the point cloud $\P$ with neural descriptors $\D$ and camera parameters $\C$, we rasterize the points with z-buffer at several resolutions, using descriptors as pseudo-colors. We  then pass the rasterizations through the U-net-like rendering network to obtain the resulting image. Our model is fit to new scene(s) by optimizing the parameters of the rendering network and the neural descriptors by backpropagating the perceptual loss function.}
%   Given a set of point clouds with registered RGB images we learn N-dimensional per-point  descriptors jointly with rendering ConvNet. During training we sample a batch of views $I$ from the database and project a corresponding pointcloud to them. For each visible point we copy its descriptor $d_i$ together with viewpoint vector to a corresponding location $s_i(C)$ on the projected image $S$.  Scene-independent  rendering network learns to map images $S$ to ground truth $I$ using perceptual loss. The descriptors $d_i$ and the rendering network are learned using backpropagation. At testing time the system can render the view for any camera position.  
%   }
  \label{fig:method}
\end{figure*}

\subsection{Rendering}

Assume that a point cloud $\P = \{p_1,p_2, \dots,\,p_N\}$ with $M$-dimensional neural descriptors attached to each point $\D = \{d_1,d_2,\dots,d_N\}$ is given, and its rendering from a new view characterized by a camera $\C$ (including both extrinsic and intrinsic parameters) needs to be obtained. In particular, assume that the target image has $W\times{}H$-sized pixel grid, and that its viewpoint is located in point $p_0$.

The rendering process first projects the points onto the target view, using descriptors as pseudo-colors, and then uses the rendering network to transform the pseudo-color image into a photorealistic RGB image. More formally, we create an $M$-channel \textit{raw image} $S(\P,\D,\C)$ of size $W\times{}H$, and for each point $p_i$ which projects to $(x, y)$ we set $S(\P,\D,\C)[[x],[y]] = d_i$ (where $[a]$ denotes a nearest integer of $a \in \mathbb{R}$). As many points may project onto the same pixel, we use z-buffer to remove occluded points. The lack of topological information in the point cloud, however, results in hole-prone representation, such that the points from the occluded surfaces and the background can be seen through the front surface (so-called \textit{bleeding} problem). This issue is traditionally addressed through splatting, i.e.\ replacing each point with a 3D disk with a radius to be estimated from data and projecting the resulting elliptic footprint of the point onto an image. We have proposed an alternative rendering scheme that does not rely on the choice of the disk radius.

% In this scheme, the rendering is performed by rasterizing each point $p_i$ into a square with the side length $r_i=\lceil\rho/\textit{depth}\rceil$ that is inversely proportional to the depth of the point w.r.t.\ the camera $\C$. The rendering is performed using OpenGL without anti-aliasing, so that the dimensions of each square are effectively rounded to the nearest integers. The z-buffer algorithm is used for superimposing these squares onto each other using their depths w.r.t.\ the camera. Let $f_i(\C)$ denote the ``footprint'' set of the point $\s_i$ resulting from such rendering, i.e.\ a set of pixels that are occupied by the rasterization of the $i$-th square after z-buffer.
% We thus create an $M$-channel \textit{raw image} $S(\P,\D,\C)$ by iterating over all footprint sets $f_i(C)$ and filling all pixels from $s_i(C)$ with the values of $d_i$ (first $M$ channels).

%\begin{equation} \label{eq:raster}
%\forall (x,y)\in \s_i:\;\; S(\P,\D,\C)[x,y] = d_i\,.
%\end{equation}

%The pixels not covered by any footprint are set to the special descriptor value $d_0 \in R^M$ (which is also learned for a particular scene).

%Finally, we use a pretrained \textit{rendering network} $\Rend_\theta$ with learnable parameters $\theta$ to map the $M$-channel raw image $S(\P,\D,\C)$ into a three-channel RGB image $I$:
%\begin{equation}
%    I(\P,\D,\C,\theta) = \Rend_\theta(\,S(\P,\D,\C)\,)\,.
%\end{equation}
%The rendering network in our case has a popular convolutional U-Net architecture~\cite{Ronneberger15} with gated convolutions~\cite{Yu18}.

%The results of this method depend on the choice of the radius parameter $\rho$ that has to somehow reflect the point density. Small $\rho$ will result in significant bleeding in the resulting raw image that needs to be addressed by the rendering network. At the same time, an excessively large $\rho$ will result in the loss of spatial detailization.  We have found that while the rendering network can handle bleeding quite well for a wide range of $\rho$ when the target viewpoints is close to the training one, or at least have a similar camera-to-scene distance. At the same time for strong closeups $\rho$ has to be increased, which may lead to detail loss.



{\bf Progressive rendering.} Rather than performing splatting, we resort to multi-scale (progressive) rendering. We thus render a point cloud $T$ times onto a pyramid of canvases of different spatial resolutions. In particular, we obtain a sequence of images $S[1],S[2]\dots S[T]$, where the $i$-th image has the size of $\frac{W}{2^t}{\times}\frac{H}{2^t}$, by performing a simple point cloud projection described above. % During rendering, we do not perform any kind of splatting, so that at each resolution the descriptor $p_i$ is rasterized onto a single pixel obtained by projecting $p_i$ onto the nearest pixel (\fig{method}).
As a result, the highest resolution raw image $S[1]$ contains the largest amount of details, but also suffers from strong surface bleeding. The lowest resolution image $S[T]$ has coarse geometric detailization, but has the least surface bleeding, while the intermediate raw images $S[2],\dots,S[T{-}1]$ achieve different detailization-bleeding tradeoffs. 

Finally, we use a \textit{rendering network} $\Rend_\theta$ with learnable parameters $\theta$ to map all the raw images into a three-channel RGB image $I$:
\begin{equation} \label{eq:render}
    I(\P,\D,\C,\theta) = \Rend_\theta(\,S[1](\P,\D,\C),\, \dots,\, S[T](\P,\D,\C) \,)\,.
\end{equation}
The rendering network in our case is based on a popular convolutional U-Net architecture~\cite{Ronneberger15}  with gated convolutions~\cite{Yu18} for better handling of a potentially sparse input. Compared to the traditional U-Net, the rendering network architecture is augmented to integrate the information from all raw images (see Fig.~\ref{fig:method}). In particular, the encoder part of the U-Net contains several downsampling layers interleaved with convolutions and non-linearities. We then concatenate the raw image $S[i]$ to the first block of the U-Net encoder at the respective resolution. Such progressive (coarse-to-fine) mechanism is reminiscent to texture mipmapping \cite{Williams83} as well as many other coarse-to-fine/varying level of details rendering algorithms in computer graphics. In our case, the rendering network provides the mechanism for implicit level of detail selection. 

The rasterization of images $S[1],\dots,S[T]$ is implemented via OpenGL. In particular U-net network has five down- and up-sampling layers. Unless noted otherwise, we set the dimensionality of descriptors to eight ($M{=}8$).


% {\bf Viewpoint-augmented rasterization.} Optionally, when rendering a raw image with a certain viewpoint $p_0$, we can augment each descriptor with a three-dimensional normalized viewpoint direction vector $v_i=\frac{p_0-p_i}{\|p_0-p_i\|}$. The resulting raw image(s) then have $M+3$ channels. The viewpoint-augmented rasterization can make modeling non-lambertian effects easier. Surprisingly, though, we observed that such non-lambertian effects can be modeled by our system even without viewpoint-augmented rasterization.


\subsection{Model creation}
\label{subsect:learning}

We now describe the fitting process in our system. We assume that during fitting $K$ different scenes are available. For the $k$-th scene the point cloud $\P^k$ as well as the set of $L_k$ training ground truth RGB images $\I^k = \{I^{k,1},I^{k,2},\dots I^{k,L_k}\}$ with known camera parameters $\{\C^{k,1},\C^{k,2},\dots \C^{k,L_k}\}$ are given. Our fitting objective $\Loss$ then corresponds to the mismatch between the rendered and the ground truth RGB images:
\begin{align} \label{eq:learn}
    \Loss(\theta,\D^1,\D^2,\dots,\D^K) = \sum_{k=1}^K\sum_{l=1}^{L_k} \Delta\left(\Rend_\theta\left(\{ S[i](\P^k,\D^k,\C^{k,l}) \}_{i=1}^T)\,\right),\;I^{k,l}\right)\,,
\end{align}
where $\D^k$ denotes the set of neural descriptors for the point cloud of the $k$-th scene, and $\Delta$ denotes the mismatch between the two images (the ground truth and the rendered one). In our implementation, we use the perceptual loss~\cite{Dosovitskiy16,Johnson16} that computes the mismatch between the activations of a pretrained VGG network~\cite{Simonyan14}. 

The fitting is performed by optimizing the loss \eq{learn} over both the parameters $\theta$ of the rendering network \textbf{and} the neural descriptors $\{\D^1,\D^2,\dots,\D^K\}$ of points in the training set of scenes. Thus, our approach learns the neural descriptors directly from data. Optimization is performed by the ADAM algorithm~\cite{Diederik14}. Note, that the neural descriptors are updated via backpropagation through \eq{render} of the loss derivatives w.r.t.\ $S(\P,\D,\C)$ onto $d_i$.

Our system is amenable for various kinds of transfer/incremental learning. Thus, while we can perform fitting on a single scene, the results for new viewpoints tend to be better when the rendering network is fitted to multiple scenes of a similar kind. In the experimental validation, unless noted otherwise, we fit the rendering network in a two stage process. We first \textit{pretrain} the rendering network on a family of scenes of a certain kind. Secondly, we fit (\textit{fine-tune}) the rendering network to a new scene. At this stage, the learning process \eq{learn} starts with zero descriptor values for the new scene and with weights of the pretrained rendering network.

% If needed, the rendering network may be fixed during fine-tuning, and only descriptor values may be updated, which keeps the rendering network ``backward-compatible'' with the corpus of the scenes it was trained on. 


% \subsection{Modeling new scenes}

% After the learning \eq{learn} is performed, a new scene can be modeled by our system given its point cloud and a set of RGB views registered with this point cloud. For example, in the case of the scene scanned with an RGBD camera, the registered RGBD views can provide both the point cloud and the RGB views. For a new scene, given a point cloud $\P'$ and a set of images $\I'=\{I'^1,I'^2,\dots, \linebreak I'^{L'}\}$ with camera parameters $\{\C'^1,\C'^2,\dots \C'^{L'}\}$, we learn the neural descriptors $\D'=\{d'_1,d'_2,\dots,d'_{N'}\}$ of the new scene, while keeping the parameters $\theta$ fixed, by optimizing the objective $\Loss'$:
% \begin{align} \label{eq:learnnew}
%     \Loss'(\D') = \sum_{l=1}^{L'} \Delta\left(\Rend_\theta\left(S(\P',\D',\C'^l)\,\right)\,,\;I'^l\right)\,.
% \end{align}
% By sharing the rendering parameters $\theta$ between the training scene and the new scene, our system is capable of better generalization resulting in a better new view synthesis. 

% Alternatively, rather than keeping the parameters $\theta$ of the rendering network fixed, we can fine-tune them to the new scene, using the pre-learned values as initializations. For some scenes, we observe modest improvements in the rendering quality of new views from such fine-tuning. In practical systems, however, it may be desirable to keep the rendering network compatible across multiple scenes (i.e.\ to have a \textit{universal} rendering network).

% \subsection{Experimental details}
% \label{sect:details}

% Our model is based on a popular U-Net~\cite{UNet} architecture with four downsampling and upsampling blocks, resulting in five rendering resolutions in the case of progressive rendering ($T=5$). We substituted max pooling layers with average pooling layers and transposed convolutions with bilinear upsampling layers. We observed that gated convolutions~\cite{Yu18} improve performance of the model on sparse input data, so normal convolutions are substituted with gated convolutions in our model. Since we use U-Net as our rendering network and learn rich point features separately, it turns out we can use lightweight network with fewer parameters. Our model has four times fewer channels in each convolutional layer than in the original architecture, resulting in 1.96M parameters. It allows us to render real-time, taking TODO ms on GeForce RTX 2080 Ti to render a 1296x968 image.

==> related.tex <==
\section{Related work}
\label{sect:related}

Our approach brings together several lines of works from computer graphics, computer vision, and deep learning communities, of which only a small subset can be reviewed due to space limitations.

\paragraph{Point-based graphics.} Using points as the modeling primitives for rendering (point-based graphics) was proposed in~\cite{Levoy85,Grossman98} and have been in active development in the 2000s~\cite{Pfister00,Zwicker01,Gross02,Kobbelt04}. The best results are obtained when each point is replaced with an oriented flat circular disk (a surfel), whereas the orientations and the radii of such disks can be estimated from the point cloud data. Multiple overlapping surfels are then rasterized and linearly combined using splatting operation~\cite{Pfister00}. More recently, \cite{Bui18} has proposed to replace linear splatting with deep convolutional network. Similarly, a rendering network is used to turn point cloud rasterizations into realistic views by \cite{Meshry19}, which rasterizes each point using its color, depth, and its semantic label. Alternatively, \cite{Pittaluga19} uses a relatively sparse point cloud such as obtained by structure-and-motion reconstruction, and rasterizes the color and the high-dimensional SIFT~\cite{Lowe04} descriptor for each point.

In our work, we follow the point-based graphics paradigm as we represent the geometry of a scene using its point cloud. However, we do not use the surface orientation, or suitable disk radii, or, in fact, even color, explicitly during rasterization. Instead, we keep a 3D point as our modeling primitive and encode all local parameters of the surface (both photometric and geometric) within neural descriptors that are learned from data. We compare this strategy with the approach of \cite{Meshry19} in the experiments.

%\subsection{RGBD scene modeling} 

%Since the introduction of Kinect, RGBD sensors have been actively used for scene modeling due to the combination of their low cost and their suitability for 3D geometry acquisition~\cite{Newcombe11,Dai17a}. Robust algorithms for RGBD-based simultaneous localization and mapping (SLAM) are now available~\cite{Sturm12,Kerl13,Endres14,Whelan15}. Most registration (SLAM) algorithms working with RGBD data construct dense volumetric scene representation, from which scene surface can be extracted e.g.\ using the marching cubes algorithm~\cite{Lorensen87}. Such surface estimation procedure, however, is limited by the resolution of the underlying volumetric grid, and in general will loose e.g.~thin details that might be present in the raw RGBD data. Our approach directly benefits from the availability of robust RGBD SLAM/registration algorithms, however it does not rely on the volumetric scene modeling and uses the point cloud assembled from the raw RGBD scans as the geometric model.

%\subsection{Surface lightfields}

%Since the inception of image-based rendering methods \cite{McMillan95,Seitz96}, several ways to parameterize the plenoptic function~\cite{McMillan95} has been proposed. Among the most efficient is the \textit{surface lightfields}~\cite{Wood00}. This parameterization samples the plenoptic function densely at the surface of the scene. Namely, for a dense set of surface elements (parameterized using surface coordinates $(u,v)$), the radiance/color along the rays along arbitrary 3D angles $\alpha$ is recorded. Most recently, the deep variant of this parameterization was proposed in \cite{Chen18}, where a fully-connected neural network accepting $(u,v,\alpha)$ as an input is used to store the surface lightfield. The network parameters are learned from a dataset of images and a surface mesh. Our approach is related to approaches based on surface lightfields, as it implicitly learns the parameterization of pointwise plenoptic function at scene surface within the neural descriptors. Unlike surface lightfields, our approach does not require scene surface modeling. Also, differently from \cite{Chen18} that outputs color value independently in each surface vertex, we use a convolutional neural network for rendering, so that the output color value at a pixel depends on multiple neural descriptors and multiple points projected to the neighborhood of this pixel.

%\subsection{Image generation with ConvNets}

%Deep splatting~\cite{Bui18} and deep surface lightfields~\cite{Chen18} are examples of a fast growing body of work that use neural networks to generate photorealistic images~\cite{Dosovitskiy15}. Generally, these works benefit greatly from the work in machine learning and image processing on generative image modeling and deep image processing, and in particular on frameworks that use adversarial learning \cite{Goodfellow14} and perceptual losses \cite{Dosovitskiy16,Johnson16} to train convolutional neural networks (ConvNets)~\cite{LeCun89} to output images (rather than to e.g.~classify them). 

%Recent works have demonstrated the ability to synthesize  high-resolution images \cite{Karras18} and to model sophisticated image \cite{Isola17,Wang18a} and video \cite{Wang18b} transformations using deep convolutional networks trained with such losses. In particular, \cite{Nalbach17} demonstrated how such \textit{pixel-to-pixel} networks can be used to replace computationally-heavy rendering and to directly transform images with rasterized material properties and normal orientations to photorealistic views. 

%Also, highly relevant to our work are methods that successfully apply deep ConvNets for image inpainting tasks \cite{Iizuka17,Liu18,Yu18}. Several modifications to the convolutional architecture with the ability to handle and fill in holes have been suggested, and in our approach we use gated convolutional layers from \cite{Yu18}.

\paragraph{Deep image based rendering.} Recent years have also seen active convergence of image-based rendering and deep learning. A number of works combine warping of preexisting photographs and the use of neural networks to combine warped images and/or to post-process the warping result. The warping can be estimated by stereo matching \cite{Flynn16}. Estimating warping fields from a single input image and a low-dimensional parameter specifying a certain motion from a low-parametric family is also possible \cite{Ganin16,Zhou16}. Other works perform warping using coarse mesh geometry, which can be obtained through multi-view stereo \cite{Hedman18,Thies18} or volumetric RGBD fusion \cite{Martin18}. Alternatively, some methods avoid explicit warping and instead use some form of plenoptic function estimation and parameterization using neural networks.  Thus, \cite{Chen18} proposes network-parameterized deep version of surface lightfields. The approach~\cite{Sitzmann19} learns neural parameterization of the plenoptic function in the form of low-dimensional descriptors situated at the nodes of a regular voxel grid and a rendering function that turns the reprojection of such desriptors to the new view into an RGB image. 

Arguably most related to ours is the deferred neural rendering (DNR) system ~\cite{Thies19}. They propose to learn \textit{neural textures} encoding the point plenoptic function at different surface points alongside the neural rendering convolutional network. Our approach is similar to \cite{Thies19}, as it also learns neural descriptors of surface elements jointly with the rendering network. The difference is that our approach uses point-based geometry representation and thus avoids the need for surface estimation and meshing. We perform extensive comparison to \cite{Thies19}, and discuss relative pros and cons of the two approaches.

